Linear Mappings of Free Algebra

For arbitrary F-algebra, in which the operation of addition is defined, I explore biring of matrices of mappings. The sum of matrices is determined by the sum in F-algebra, and the product of matrices is determined by the product of mappings. The system of equations, whose matrix is a matrix of mappings, is called a system of additive equations. I considered the methods of solving system of additive equations. As an example, I consider the solution of a system of linear equations over the complex field provided that the equations contain unknown quantities and their conjugates. Linear mappings of algebra over a commutative ring preserve the operation of addition in algebra and the product of elements of the algebra by elements of the ring. The representation of tensor product A\otimes A in algebra A generates the set of linear transformations of algebra A. The results of this research will be useful for mathematicians and physicists who deal with different algebras.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Greiner Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem
{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов, Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин,
Элементы теории функций и функционального анализа,
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том 1, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

%\BiblioItem{Kleyn} http://www.geocities.com/aleks\_kleyn/Derivative/Derivative.htm

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{Muller}
{
Holger Muller et al.,
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators,
\href{http://prola.aps.org/searchabstract/PRL/v91/i2/e020401}{Phys. Rev. Lett. 91, 020401} (2003),
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2000)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem
{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
I. Gelfand and V. Retakh, Determinants of Matrices over Noncommutative Rings, Funct.
Anal. Appl. 25 (1991), no. 2, 91-102
}%

\BiblioItem{Gelfand Retakh 1992}
{
I. Gelfand and V. Retakh, A Theory of Noncommutative Determinants and Characteristic
Functions of Graphs, Funct. Anal. Appl. 26 (1992), no. 4, 1-20
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная $\mathfrak{F}$\Hyph алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление $\mathfrak{F}$\Hyph алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:q-alg/1004.3007} (2010)
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М. Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fihtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Complex.Number.Russian.tex <==
%auto-ignore

\input{Complex.Number.Eq}

\section{Линейная функция комплексного поля}
\label{section: Linear Function of Complex Field}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\label{theorem: complex field over real field}
Рассмотрим поле комплексных чисел $C$ как двумерную алгебру над полем действительных чисел.
Положим
\ShowEq{basis of complex field}
базис алгебры $C$.
Тогда в этом базисе произведение имеет вид
\ShowEq{product of complex field}
и структурные константы имеют вид
\ShowEq{structural constants of complex field}
Матрица линейной функции
\[
y^{\gi i}=x^{\gi j}f_{\gi j}^{\gi i}
\]
поля комплексных чисел над полем действительных чисел
удовлетворяет соотношению
\begin{align}
\label{eq: complex field over real field, 0}
f_{\gi 0}^{\gi 0}&=f_{\gi 1}^{\gi 1}
\\
\label{eq: complex field over real field, 1}
f_{\gi 0}^{\gi 1}&=-f_{\gi 1}^{\gi 0}
\end{align}
\end{theorem}
\begin{proof}
Равенства
\EqRef{product of complex field} и
\EqRef{structural constants of complex field}
следуют из равенства $i^2=-1$.
Пользуясь равенством
\xEqRef{0812.4763}{eq: linear map over field, division ring, relation}
получаем соотношения
\ShowEq{complex field over real field}
Из равенств
\EqRef{complex field over real field, 0, 0} и
\EqRef{complex field over real field, 0, 1}
следует \EqRef{complex field over real field, 0}.
Из равенств
\EqRef{complex field over real field, 1, 0} и
\EqRef{complex field over real field, 1, 1}
следует \EqRef{complex field over real field, 1}.
\end{proof}

\ePrints{0701.238,1003.1544}
\ifx\Semafor\ValueOff
\begin{theorem}[Уравнения Коши\Hyph Римана]
Если матрица
\ShowEq{Jacobian of map of complex variable}
является матрицей Якоби функции комплексного переменного
\[
x=x^{\gi 0}+x^{\gi 1}i\rightarrow y=y^{\gi 0}(x^{\gi 0},x^{\gi 1})+y^{\gi 1}(x^{\gi 0},x^{\gi 1})i
\]
над полем действительных чисел,
то
\ShowEq{Cauchy Riemann equations, complex field, 1}
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: complex field over real field}.
\end{proof}

\begin{theorem}
Производная функции комплексного переменного удовлетворяет равенству
\ShowEq{Cauchy Riemann equations, complex field, 2}
\end{theorem}
\begin{proof}
Равенство
\ShowEq{Cauchy Riemann equations, complex field, 2, 1}
следует из равенств
\EqRef{Cauchy Riemann equations, complex field, 1}.
\end{proof}

Равенство \EqRef{Cauchy Riemann equations, complex field, 2}
эквивалентно равенству
\ShowEq{Cauchy Riemann equations, complex field, 3}
\ifx\texFuture\Defined
Производная Гато функции комплексного переменного является
полным дифференциалом и имеет вид
\ShowEq{Gateaux derivative, complex field}
где $dx$, $dy\in R$.
Поэтому символическое уравнение
\ShowEq{Cauchy Riemann equations, Gateaux derivative, complex field}
не выражает связь производной Гато с уравнения Коши\Hyph Римана.
\fi
\fi

\section{Алгебра кватернионов}

В этой статье я рассматриваю множество кватернионных алгебр,
определённых в \citeBib{Izrail M. Gelfand: Quaternion Groups}.

\begin{definition}
Пусть $F$ - поле.
Расширение $F(i,j,k)$ поля $F$ называется
\AddIndex{алгеброй
\symb{E(F,a,b)}1{quaternion algebra over the field}
кватернионов над полем $F$}{quaternion algebra over the field}\footnote{Я
буду следовать определению из \citeBib{Izrail M. Gelfand: Quaternion Groups}.},
если произведение в алгебре $E$ определено согласно правилам
\ShowEq{product in E(F,a,b), table}
где $a$, $b\in F$, $ab\ne 0$.

Элементы алгебры $E(F,a,b)$ имеют вид
\[
x=x^{\gi 0}+x^{\gi 1}i+x^{\gi 2}j+x^{\gi 3}k
\]
где $x^{\gi i}\in F$, $\gi i=\gi 0$, $\gi 1$, $\gi 2$, $\gi 3$.
Кватернион
\[
\overline x=x^{\gi 0}-x^{\gi 1}i-x^{\gi 2}j-x^{\gi 3}k
\]
называется сопряжённым кватерниону $x$.
Мы определим
\AddIndex{норму кватерниона}{norm of quaternion}
$x$ равенством
\ShowEq{norm of quaternion E(F,a,b)}
Из равенства \EqRef{norm of quaternion E(F,a,b)} следует, что
$E(F,a,b)$ является алгеброй с делением только когда $a<0$, $b<0$.
Тогда мы можем пронормировать базис так, что $a=-1$, $b=-1$.

Мы будем обозначать символом
\ShowEq{quaternion division algebra over the field}
алгебру $E(F,-1,-1)$
кватернионов с делением над полем $F$.
Произведение в алгебре $E(F)$ определено согласно правилам
\begin{equation}
\begin{array}{c|ccc}
&i&j&k\\
\hline
i&-1&k&-j\\
j&-k&-1&i\\
k&j&-i&-1\\
\end{array}
\label{eq: product of quaternions}
\end{equation}
\qed
\end{definition}
В алгебре $E(F)$ норма кватерниона имеет вид
\begin{equation}
\label{eq: norm of quaternion}
|x|^2=x\overline x=(x^{\gi 0})^2+(x^{\gi 1})^2+(x^{\gi 2})^2+(x^{\gi 3})^2
\end{equation}
При этом обратный элемент имеет вид
\begin{equation}
\label{eq: inverce quaternion}
x^{-1}=|x|^{-2}\overline x
\end{equation}

\symb{H}0{quaternion algebra over real field}
Мы будем полагать $\ShowSymbol{quaternion algebra over real field}=E(R,-1,-1)$.

Внутренний автоморфизм алгебры кватернионов $H$\footnote{См.
\citeBib{Hamilton papers 3}, с. 643.}
\ShowEq{Quaternion Rotation}
описывает вращение вектора с координатами $x$, $y$, $z$.
Если $q$ записан в виде суммы скаляра и вектора
\ShowEq{Quaternion Rotation, 1}
то \EqRef{Quaternion Rotation} описывает вращение
вектора $(x,y,z)$ вокруг вектора $(a,b,c)$ на угол $2\alpha$.



==> Convention.Russian.tex <==
%auto-ignore
\input{Convention.Eq}

\section{Соглашения}

\begin{enumerate}

\ePrints{0812.4763,0906.0135,0908.3307,0909.0855,0912.3315,1003.1544}
\Items{1006.2597}
\ifx\Semafor\ValueOn
\item Функция и отображение - синонимы. Однако существует
традиция соответствие между кольцами или векторными
пространствами называть отображением, а отображение
поля действительных чисел или алгебры кватернионов называть функцией.
Я тоже следую этой традиции,
хотя встречается текст, в котором неясно, какому термину надо
отдать предпочтение.
%Однако мы можем рассматривать свободную
%алгебру как векторное пространство над полем.
%Так как нежелательно одно и тоже соответствие называть то функцией, то
%отображением, я буду пользоваться термином линейная функция алгебры.
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1001.4852}
\Items{1003.1544}
\ifx\Semafor\ValueOn
\item
В любом выражении, где появляется индекс, я предполагаю,
что этот индекс может иметь внутреннюю структуру.
Например, при рассмотрении алгебры $A$ координаты $a\in A$
относительно базиса $\Basis e$ пронумерованы индексом $i$.
Это означает, что $a$ является вектором. Однако, если $a$
является матрицей, нам необходимо два индекса, один нумерует
строки, другой - столбцы. В том случае, когда мы уточняем структуру
индекса, мы будем начинать индекс с символа $\cdot$ в соответствующей
позиции.
Например, если я рассматриваю матрицу $a^i_j$ как элемент векторного
пространства, то я могу записать элемент матрицы в виде $a^{\cdot}{}^i_j$.
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1006.2597}
\ifx\Semafor\ValueOn
\item
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $s$.
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855}
\ifx\Semafor\ValueOn
\item
Тело $D$ можно рассматривать как $D$\Hyph векторное пространство
размерности $1$. Соответственно этому, мы можем изучать не только
гомоморфизм тела $D_1$ в тело $D_2$, но и линейное отображение тел.
При этом подразумевается, что отображение мультипликативно над
максимально возможным полем. В частности, линейное отображение
тела $D$ мультипликативно над центром $Z(D)$. Это не противоречит
определению линейного отображения поля, так как для поля $F$ справедливо
$Z(F)=F$.
Если поле $F$ отлично
от максимально возможного, то я это явно указываю в тексте.
\fi

\ePrints{0912.4061}
\ifx\Semafor\ValueOn
\item
Для данного поля $F$, если не оговорено противное,
мы будем рассматривать конечномерную $F$\Hyph алгебру.
%без делителей нуля.
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307}
\ifx\Semafor\ValueOn
\item
Несмотря на некоммутативность произведения многие утверждения
сохраняются, если заменить например правое представление на
левое представление или правое векторное пространство на левое
векторное пространство.
Чтобы сохранить эту симметрию в формулировках теорем
я пользуюсь симметричными обозначениями.
Например, я рассматриваю \Ds векторное пространство
и \sD векторное пространство.
Запись \Ds векторное пространство можно прочесть
как D\Hyph star\Hyph векторное пространство либо
как левое векторное пространство.
Запись \Ds линейно зависимые векторы можно прочесть
как D\Hyph star\Hyph линейно зависимые векторы либо
как векторы, линейно зависимые слева.
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597}
\ifx\Semafor\ValueOn
\item Пусть $A$ - свободная конечно
мерная алгебра.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
Однако в алгебре не принято использовать векторные обозначения.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}

\item Если свободная конечномерная алгебра имеет единицу,
то мы будем отождествлять
вектор базиса $\Vector e_{\gi 0}$ с единицей алгебры.
\fi

\ePrints{0906.0135,0912.3315}
\ifx\Semafor\ValueOn
\item В \citeBib{Cohn: Universal Algebra}
произвольная операция алгебры обозначена буквой $\omega$,
и $\Omega$ - множество операций некоторой универсальной алгебры.
Соответственно, универсальная алгебра с множеством операций
$\Omega$ обозначается $\Omega$\Hyph алгебра.
Аналогичные обозначения мы видим в
\citeBib{Burris Sankappanavar} с той небольшой разницей,
что операция в алгебре обозначена буквой $f$
и $\mathcal F$ - множество операций.
Я выбрал первый вариант обозначений, так как в этом случае
легче видно, где я использую операцию.
\fi

\ePrints{0906.0135,0912.3315}
\ifx\Semafor\ValueOn
\item
Так как число универсальных алгебр в башне представлений переменно,
то мы будем пользоваться векторными обозначениями для башни
представлений. Множество
$(A_1,...,A_n)$ $\Omega_i$\Hyph алгебр $A_i$, $i=1$, ..., $n$
мы будем обозначать $\Vector A$. Множество представлений
$(f_{1,2},...,f_{n-1,n})$ этих алгебр мы будем обозначать $\Vector f$.
Так как разные алгебры имеют разный тип, мы также
будем говорить о множестве $\Vector{\Omega}$\Hyph алгебр.
По отношению к множеству $\Vector A$
мы также будем пользоваться матричными обозначениями, предложенными
в разделе \xRef{0701.238}{section: Concept of Generalized Index}.
Например, символом $\Vector A_{[1]}$ мы будем обозначать
множество $\Vector{\Omega}$\Hyph алгебр $(A_2,...,A_n)$.
В соответствующем обозначении $(\Vector A_{[1]},\Vector f)$ башни
представлений подразумевается, что $\Vector f=(f_{2,3},...,f_{n-1,n})$.

\item Так как мы пользуемся векторными обозначениями для элементов
башни представлений, необходимо соглашение о записи операций.
Предполагается, что операции выполняются покомпонентно. Например,
\ShowEq{vector notation in tower of representations}
\fi

\ePrints{0912.3315}
\ifx\Semafor\ValueOn
\item
Я считаю диаграммы отображений важным инструментом. Однако временами возникает
желание увидеть диаграмму трёх мерной, что увеличило бы её выразительную
мощность. Кто знает какие сюрпризы готовит будущее.
В 1992 на конференции в Казани я рассказывал своим коллегам
какие преимущества имеет компьютерная подготовка статей.
Спустя 8 лет из письма из Казани я узнал, что теперь можно
готовить статьи с помощью LaTeX.
\fi

\ePrints{1001.4852,1003.1544,1006.2597}
\ifx\Semafor\ValueOn
\item Если в некотором выражении используется несколько
операций, среди которых есть операция $\circ$, то предполагается,
что операция $\circ$ выполняется первой.
Ниже приведен пример эквивалентных выражений.
\ShowEq{list circ expressions}
\fi

\item
Без сомнения, у читателя моих статей могут быть вопросы,
замечания, возражения. Я буду признателен любому отзыву.

\end{enumerate}



==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%1%1%1-rcd форма
   {$1$-\rcd форма}%
   {1-rcd form, vector spaces}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%3%A%a b-CR квазидетерминант
   {$(^a_b)$\hyph \CR квазидетерминант}%
   {a b cr-quasideterminant}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) mapping}%
\Index%581%A%Arc  линейно зависимые векторы
   {$A\RCstar$\Hyph  линейно зависимые векторы}%
   {linearly dependent, A vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%580%A%Arc линейно независимые векторы
   {$A\RCstar$\Hyph линейно независимые векторы}%
   {linearly independent, A vector space}%
\Index%575%A%Astar векторное пространство
   {$A\star$\Hyph векторное пространство}%
   {Astar vector space}%
\Index%583%A%Astar линейное отображение векторных пространств
   {$A\star$\Hyph линейное отображение векторных пространств}%
   {Astar linear map of vector spaces}%
\Index%579%A%Astar-произведение вектора на скаляр
   {$A\star$\hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, vector space}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение матриц
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%13%C%crd производная Гато отображения \Vector f D-векторного пространства \Vector V в D-векторное пространство \Vector W
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%23%D%d аффинное пространство
   {$D$\Hyph аффинное пространство}%
   {d affine space}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%20%D%Drc  линейно зависимые векторные поля
   {\Drc  линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%111%D%drc аффинный базис
   {\drc аффинный базис}%
   {drc affine basis, division ring}%
\Index%26%D%Drc базис в векторном расслоении
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index%16%D%drc базис векторного пространства r строк
   {\drc базис векторного пространства \subs строк}%
   {drc basis, r rows vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%19%D%drc векторное пространство r строк
   {\drc векторное пространство \subs строк}%
   {subs rows drc vector space}%
\Index%30%D%drc вектор-функция
   {\drc вектор\hyph функция}%
   {drc vector function}%
\Index%33%D%Drc линейно независимые векторные поля
   {\Drc линейно независимые векторные поля}%
   {linearly independent vector fields}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%70%D%drc представление группы
   {\drc представление группы}%
   {drc linear representation of group}%
\Index%38%D%drc производная Гато отображения \Vector f D- векторного пространства \Vector V в D- векторное пространство \Vector W
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%42%D%Dstar компонента координат вектора \Vector r
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%40%D%Dstar-векторное пространство
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%44%D%Dstar-произведение вектора на скаляр
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\Index%25%D%rcd базис в векторном пространстве c строк
   {\rcd базис в векторном пространстве \sups строк}%
   {rcd basis, c rows vector space}%
\Index%32%D%rcd линейная оболочка в векторном пространстве
   {\rcd линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index%49%R%drc базис, дуальный rcd базису в векторном пространстве
   {\drc базис, дуальный \rcd базису в векторном пространстве}%
   {basis dual to basis, rcd vector space}%
\Index%4%R%j i-RC квазидетерминант
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главный минор
   {\RC главный минор}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение матриц
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%600%R%RCcirc вырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph вырожденная матрица $\mathcal A(A)$\Hyph отображений}%
   {RCcirc singular matrix of A(A) mappings}%
\Index%599%R%RCcirc вырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph вырожденная матрица эндоморфизмов}%
   {RCcirc singular matrix of endomorphisms}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph невырожденная матрица $A(A)$\Hyph отображений}%
   {RCcirc nonsingular matrix of A(A) mappings}%
\Index%598%R%RCcirc невырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph невырожденная матрица эндоморфизмов}%
   {RCcirc nonsingular matrix of endomorphisms}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%21%R%rcd  линейно зависимые векторы
   {\rcd  линейно зависимые векторы}%
   {linearly dependent, vector space}%
\Index%22%R%rcd автоморфизм векторного пространства
   {\rcd автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%24%R%rcd базис в векторном пространстве
   {\rcd базис в векторном пространстве}%
   {rcd basis, vector space}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%29%R%rcd векторное пространство c строк
   {\rcd векторное пространство \sups строк}%
   {sups rows rcd vector space}%
\Index%31%R%rcd изоморфизм векторных пространств
   {\rcd изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%34%R%rcd линейно независимые векторы
   {\rcd линейно независимые векторы}%
   {linearly independent, vector space}%
\Index%35%R%rcd линейное отображение векторных пространств
   {\rcd линейное отображение векторных пространств}%
   {rcd linear map of vector spaces}%
\Index%37%R%rcd линейным Tstar- представление группы
   {\rcd линейным \Ts представление группы}%
   {rcd linear Tstar representation of group}%
\Index%71%R%Rstar- модуль
   {$R\star$\Hyph модуль}%
   {Rstar-module}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index%77%S%Dstar- произведением rcd линейного отображения A на скаляр
   {$D\star$\Hyph произведением \rcd линейного отображения $A$ на скаляр}%
   {Dstar product of rcd linear map over scalar}%
\Index%73%S%RCstarS,RCstarT- линейное отображение векторных пространств
   {$(\RCstar S,\RCstar T)$\Hyph линейное отображение векторных пространств}%
   {rcs rct linear map of vector spaces}%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%586%S%star A- product of Astar linear map over scalar
   {$\star A$\Hyph произведением $A\star$\Hyph линейного отображения на скаляр}%
   {starA product of Astar linear map over scalar}%
\Index%78%S%star D-векторное пространство
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%75%S%starD компонента координат вектора \Vector r
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%82%S%starT- представление Omega1 алгебры A в Omega2 алгебре M
   {\sT представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {starT representation of algebra}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%85%S%starT- преобразование
   {\sT преобразование}%
   {starT transformation}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%80%S%starT- сдвиг
   {\sT сдвиг}%
   {starT shift}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%87%T%Tstar- векторное пространство матриц
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index%88%T%Tstar- линейная комбинация векторов
   {\Ts линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index%90%T%Tstar- представление Omega1 алгебры A в Omega2 алгебре M
   {\Ts представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {Tstar representation of algebra}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%92%T%Tstar- преобразование
   {\Ts преобразование}%
   {Tstar transformation}%
\Index%93%T%Tstar- преобразование расслоения
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\Index%89%T%Tstar- сдвиг
   {\Ts сдвиг}%
   {Tstar shift}%
\SetIndexSpace%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%94%А%автоморфизм представления F алгебры
   {автоморфизм представления $\mathfrak{F}$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%99%А%активное starT- представление
   {активное \sT представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%569%А%активное представление лупы в многообразии базисов
   {активное представление лупы $\mathfrak A(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%106%А%антигомоморфизм расслоенных групп
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%616%А%ассоциатор R алгебры
   {ассоциатор $R$\Hyph алгебры}%
   {associator of algebra}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%115%Б%базис векторного пространства
   {базис векторного пространства}%
   {Basis}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%117%Б%базовый вектор представления группы Ли
   {базовый вектор представления группы Ли}%
   {basis vector of representation of Lie group}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Vector{\Omega}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%121%Б%бесконечно малый генератор
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index%123%В%вектор Килинга второго рода
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%130%В%вырожденное линейное отображение D- векторного пространства
   {вырожденное линейное отображение $D$\Hyph векторного пространства}%
   {singular linear map, D vector space}%
\Index%131%В%вырожденное линейное отображение тела
   {вырожденное линейное отображение тела}%
   {singular linear map, division ring}%
\SetIndexSpace%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\mathcal{E}$}%
   {Cartesian power n of bundle E}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%156%Д%дифференциал Гато второго порядка отображения \Vector f
   {дифференциал Гато второго порядка отображения $\Vector f$}%
   {Gateaux differential of Second Order, D vector space}%
\Index%155%Д%дифференциал Гато второго порядка отображения f
   {дифференциал Гато второго порядка отображения $f$}%
   {Gateaux differential of Second Order, division ring}%
\Index%632%Д%дифференциал Гато второго порядка отображения f алгебры
   {дифференциал Гато второго порядка отображения $f$ алгебры}%
   {Gateaux differential of Second Order, algebra}%
\Index%157%Д%дифференциал Гато отображения \Vector f нормированного D- векторного пространства V в нормированное D- векторное пространство W
   {дифференциал Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux differential of map, D vector space}%
\Index%158%Д%дифференциал Гато отображения f
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, division ring}%
\Index%628%Д%дифференциал Гато отображения алгебры
   {дифференциал Гато отображения $f$ алгебры}%
   {Gateaux differential of map, algebra}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\SetIndexSpace%
\Index%576%З%закон ассоциативности для Astar- векторного пространства
   {закон ассоциативности для $A\star$\Hyph векторного пространства}%
   {associative law, Astar vector space}%
\Index%585%З%закон ассоциативности для Astar линейных отображений векторных пространств
   {закон ассоциативности для $A\star$\Hyph линейных отображений векторных пространств}%
   {associative law for Astar linear mappings of vector spaces}%
\Index%162%З%закон ассоциативности для Drc линейных отображений векторных расслоений
   {закон ассоциативности для \Drc линейных отображений векторных расслоений}%
   {associative law for drc linear maps of vector bundles}%
\Index%163%З%закон ассоциативности для Dstar- векторного пространства
   {закон ассоциативности для $D\star$\Hyph векторного пространства}%
   {associative law, Dstar vector space}%
\Index%164%З%закон ассоциативности для Dstar- векторных полей
   {закон ассоциативности для $\mathcal D\star$\Hyph векторных полей}%
   {associative law, Dstar vector fields}%
\Index%161%З%закон ассоциативности для rcd линейных отображений векторных пространств
   {закон ассоциативности для \rcd линейных отображений векторных пространств}%
   {associative law for rcd linear maps of vector spaces}%
\Index%165%З%закон ассоциативности для ковариантного starT- представления
   {закон ассоциативности для ковариантного \sT представления}%
   {associative law for covariant starT representation}%
\Index%166%З%закон ассоциативности для ковариантного Tstar- представления
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for covariant Tstar representation}%
\Index%167%З%закон ассоциативности для парных представлений
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index%168%З%закон ассоциативности произведения расслоенных соответствий
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index%577%З%закон дистрибутивности для Astar- векторного пространства
   {закон дистрибутивности для $A\star$\Hyph векторного пространства}%
   {distributive law, Astar vector space}%
\Index%169%З%закон дистрибутивности для Dstar- векторного пространства
   {закон дистрибутивности для $D\star$\Hyph векторного пространства}%
   {distributive law, Dstar vector space}%
\Index%170%З%закон дистрибутивности для Dstar- векторных полей
   {закон дистрибутивности для $\mathcal D\star$\Hyph векторных полей}%
   {distributive law, Dstar vector fields}%
\Index%578%З%закон унитарности для Astar- векторного пространства
   {закон унитарности для $A\star$\Hyph векторного пространства}%
   {unitarity law, Astar vector space}%
\Index%171%З%закон унитарности для Dstar- векторного пространства
   {закон унитарности для $D\star$\Hyph векторного пространства}%
   {unitarity law, Dstar vector space}%
\Index%172%З%закон унитарности для Dstar- векторных полей
   {закон унитарности для $\mathcal D\star$\Hyph векторных полей}%
   {unitarity law, Dstar vector fields}%
\SetIndexSpace%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%176%К%категория Tstar- представлений Omega1 алгебры A
   {категория \Ts представлений $\Omega$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Index%177%К%категория Tstar- представлений Omega1 алгебры из категории A
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of mappings}%
\Index%184%К%ковариантное starT- представление группы
   {ковариантное \sT представление группы}%
   {covariant starT representation of group}%
\Index%185%К%ковариантное starT- представление расслоенной группы
   {ковариантное \sT представление расслоенной группы}%
   {covariant starT representation of fibered group}%
\Index%186%К%ковариантное Tstar- представление группы
   {ковариантное \Ts представление группы}%
   {covariant Tstar representation of group}%
\Index%187%К%ковариантное Tstar- представление расслоенной группы
   {ковариантное \Ts представление расслоенной группы}%
   {covariant Tstar representation of fibered group}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%614%К%коммутатор R алгебры
   {коммутатор $R$\Hyph алгебры}%
   {commutator of algebra}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%192%К%компонента линейного отображения D- векторного пространчства
   {компонента линейного отображения $D$\Hyph векторного пространчства}%
   {component of linear map, D vector space}%
\Index%193%К%компонента линейного отображения f тела
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Index%194%К%компонента полилинейного отображения \Vector A
   {компонента полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Index%195%К%компонента полилинейного отображения тела
   {компонента полилинейного отображения тела}%
   {component of polylinear map, division ring}%
\Index%196%К%компонента производной Гато второго порядка отображения \Vector f(\Vector x)
   {компонента производной Гато второго порядка отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Index%633%К%компонента производной Гато второго порядка отображения f(x) алгебры
   {компонента производной Гато второго порядка отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of Second Order, algebra}%
\Index%197%К%компонента производной Гато второго порядка отображения тела
   {компонента производной Гато второго порядка отображения тела}%
   {component of Gateaux derivative of Second Order, division ring}%
\Index%199%К%компонента производной Гато отображения \Vector f(\Vector x)
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space}%
\Index%198%К%компонента производной Гато отображения f(x)
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, division ring}%
\Index%629%К%компонента производной Гато отображения f(x) алгебры
   {компонента производной Гато отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of map, algebra}%
\Index%202%К%контравариантное starT- представление группы
   {контравариантное \sT представление группы}%
   {contravariant starT representation of group}%
\Index%200%К%контравариантное starT- представление расслоенной группы
   {контравариантное \sT представление расслоенной группы}%
   {contravariant starT representation of fibered group}%
\Index%201%К%контравариантное Tstar- представление группы
   {контравариантное \Ts представление группы}%
   {contravariant Tstar representation of group}%
\Index%203%К%контравариантное Tstar- представление расслоенной группы
   {контравариантное \Ts представление расслоенной группы}%
   {contravariant Tstar representation of fibered group}%
\Index%204%К%координатная матрица вектора в rcd базисе
   {координатная матрица вектора в \rcd базисе}%
   {coordinate matrix of vector in rcd basis}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов в векторном пространстве dcr строк
   {координатная матрица множества векторов в векторном пространстве \dcr строк}%
   {coordinate matrix of set of vectors, dcr vector space}%
\Index%207%К%координатная матрица множества векторов в векторном пространстве rcd строк
   {координатная матрица множества векторов в векторном пространстве \rcd строк}%
   {coordinate matrix of set of vectors, rcd vector space}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%210%К%координатное Drc векторное расслоение
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%214%К%координатный rcd изоморфизм
   {координатный \rcd изоморфизм}%
   {coordinate rcd isomorphism}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%323%К%координаты автоморфизма представления
   {координаты автоморфизма представления}%
   {coordinates of automorphism of representation}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора в rcd базисе
   {координаты вектора в \rcd базисе}%
   {coordinates of vector in rcd basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometric object, coordinate vector space}%
\Index%222%К%координаты множества векторов в dcr векторном пространстве
   {координаты множества векторов в \dcr векторном пространстве}%
   {coordinates of set of vectors, dcr vector space}%
\Index%223%К%координаты множества векторов в rcd векторном пространстве
   {координаты множества векторов в \rcd векторном пространстве}%
   {coordinates of set of vectors, rcd vector space}%
\Index%571%К%координаты пассивного отображения многообразия базисов представления
   {координаты пассивного отображения многообразия базисов представления}%
   {coordinates of passive map of basis manifold of representation}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%558%К%координаты элемента относительно множества
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%230%Л%левостороннее ковариантное представление группы
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation of group}%
\Index%231%Л%левостороннее контравариантное представление группы
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation of group}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%237%Л%левый модуль
   {левый модуль}%
   {left module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index%98%Л%линейнное отображение тела, порождённое отображением G
   {линейное отображение тела, порождённое отображением $G$}%
   {linear map generated by map, division ring}%
\Index%608%Л%линейное отображение  R_1 модуля в R_2 модуль
   {линейное отображение  $R_1$\Hyph модуля $A_1$ в $R_2$\Hyph модуль $A_2$}%
   {linear mapping of R_1 module into R_2 module}%
\Index%242%Л%линейное отображение D- векторных пространств над полем F
   {линейное отображение $D$\Hyph векторных пространств над полем $F$}%
   {linear map over field, vector space}%
\Index%610%Л%линейное отображение R алгебры в R алгебру
   {линейное отображение $R$\Hyph алгебры $A_1$ в $R$\Hyph алгебру $A_2$}%
   {linear mapping of R algebras}%
\Index%613%Л%линейное отображение R модуля в R модуль
   {линейное отображение $R$\Hyph модуля $A_1$ в $R$\Hyph модуль $A_2$}%
   {linear mapping of R modules}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear mapping of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\Index%568%Л%лупа автоморфизмов представления
   {лупа автоморфизмов представления}%
   {loop of automorphisms of representation}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%584%М%матрица Astar линейного отображения
   {матрица $A\star$\Hyph линейного отображения}%
   {matrix of Astar linear map}%
\Index%251%М%матрица rcd линейного отображения
   {матрица \rcd линейного отображения}%
   {matrix of rcd linear map}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear mappings}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of mappings}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов H алгебры
   {матрица эндоморфизмов $\mathfrak{H}$\Hyph алгебры}%
   {matrix of endomorphisms of H algebra}%
\Index%527%М%матрица Якоби Гато отображения D- векторного пространства
   {матрица Якоби\Hyph Гато отображения $D$\Hyph векторного пространства}%
   {Jacobi Gateaux matrix of map, D vector space}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%257%М%многообразие drc базисов аффинного пространства
   {многообразие \drc базисов аффинного пространства}%
   {drc Basis Manifold, Affine Space, division ring}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%261%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%331%М%множество образующих подпредставления
   {множество образующих подпредставления}%
   {generating set of subrepresentation}%
\Index%332%М%множество образующих представления
   {множество образующих представления}%
   {generating set of representation}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни Tstar- представлений в башню Tstar- представлений
   {морфизм из башни \Ts представлений в башню \Ts представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\mathcal{F}$ в $\mathcal{G}$}%
   {morphism of fibered representations from f into g}%
\SetIndexSpace%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor, algebra}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%313%Н%непрерывная функция над алгебро1
   {непрерывная функция над $D$\Hyph алгебро1}%
   {continuous function, algebra}%
\Index%280%Н%непрерывная функция тела
   {непрерывная функция тела}%
   {continuous function, division ring}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%346%Н%норма на D- алгебре
   {норма на $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%284%Н%норма на теле
   {норма на теле}%
   {absolute value on division ring}%
\Index%285%Н%норма отображения  тела
   {норма отображения  тела}%
   {norm of map, division ring}%
\Index%286%Н%норма отображения \Vector A нормированного D-векторного пространства
   {норма отображения $\Vector A$ нормированного $D$\hyph векторного пространства}%
   {norm of map, D vector space}%
\Index%314%Н%норма отображения в D- алгебру
   {норма отображения в $D$\Hyph алгебру}%
   {norm of map, algebra}%
\Index%343%Н%нормированная D- алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%287%Н%нормированное D- векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\SetIndexSpace%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map, division ring}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство группы
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%304%О%орбита Tstar- представления группы
   {орбита \Ts представления группы}%
   {orbit of Tstar  representation of group}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормальный базис
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормальный базис
   {ортонормальный базис}%
   {Orthonornal Basis, division ring}%
\Index%638%О%ортонормированый базис в пространстве Минковского
   {ортонормированый базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%587%П%парные представления ассоциативной алгебры
   {парные представления ассоциативной алгебры}%
   {twin representations of associative algebra}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное starT- представление
   {пассивное \sT представление}%
   {passive starT representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%345%П%полиалинейное косо симметричное отображение
   {полиалинейное косо симметричное отображение}%
   {polylinear map skew symmetric, division ring}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%342%П%полилинейное отображение (n)-D-векторных пространств
   {полилинейное отображение $(n)$\hyph $D$\hyph векторных пространств}%
   {polylinear map of D vector spaces}%
\Index%609%П%полилинейное отображение алгебр
   {полилинейное отображение алгебр}%
   {polylinear map of algebras}%
\Index%621%П%полилинейное отображение модулей
   {полилинейное отображение модулей}%
   {polylinear map of modules}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric, division ring}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%351%П%последовательность Коши в нормированное теле
   {последовательность Коши в нормированное теле}%
   {Cauchy sequence, valued division ring}%
\Index%271%П%последовательность Коши в нормированном алгебре
   {последовательность Коши в нормированном алгебрае}%
   {Cauchy sequence, normed algebra}%
\Index%241%П%последовательность Коши в нормированном кольце
   {последовательность Коши в нормированном кольце}%
   {Cauchy sequence, normed ring}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%355%П%правостороннее ковариантное представление группы
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation of group}%
\Index%356%П%правостороннее контравариантное представление группы
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation of group}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%361%П%правый модуль
   {правый модуль}%
   {right module}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%460%П%предел последовательности в нормированной алгебре
   {предел последовательности в нормированной алгебре}%
   {limit of sequence, normed algebra}%
\Index%467%П%предел последовательности в нормированном кольце
   {предел последовательности в нормированном кольце}%
   {limit of sequence, normed ring}%
\Index%364%П%предел последовательности в нормированном теле
   {предел последовательности в нормированном теле}%
   {limit of sequence, valued division ring}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\mathcal{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%384%П%принцип инвариантности
   {принцип инвариантности}%
   {invariance principle}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\mathcal{E}$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%390%П%произведение групп
   {произведение групп}%
   {product of groups}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%395%П%произведением объектов в категории
   {произведением объектов в категории}%
   {product of objects in category}%
\Index%396%П%производная Гато второго порядка отображения f
   {производная Гато второго порядка отображения $f$}%
   {Gateaux derivative of Second Order, division ring}%
\Index%626%П%производная Гато второго порядка отображения алгебры
   {производная Гато второго порядка отображения алгебры}%
   {Gateaux derivative of Second Order, algebra}%
\Index%397%П%производная Гато отображения f
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, division ring}%
\Index%398%П%производная Гато отображения Vector f нормированого D- векторного пространства Vector V в нормированное D- векторное пространство Vector W
   {производная Гато отображения $\Vector f$ нормированого $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux derivative of map, D vector space}%
\Index%627%П%производная Гато отображения алгебры
   {производная Гато отображения алгебры}%
   {Gateaux derivative of map, algebra}%
\Index%399%П%производная Гато порядка n отображения \Vector f
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Index%634%П%производная Гато порядка n отображения f алгебры
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, algebra}%
\Index%400%П%производная Гато порядка n отображения f тела
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит Tstar- представления
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%412%П%прямое произведение Tstar- представлений группы
   {прямое произведение \Ts представлений группы}%
   {direct product of Tstar representations of group}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\mathcal{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%441%С%свободное Tstar- представление группы
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%612%С%свободный модуль над кольцом
   {свободный модуль над кольцом}%
   {free module over ring}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%453%С%смешанная частная производная Гато отображения f^j по переменным v^i, v^j
   {смешанная частная производная Гато отображения $f^j$ по переменным $v^i$, $v^j$}%
   {Gateaux partial derivative of Second Order, D vector space}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%456%С%стандартная F- компонента линейного отображения f
   {стандартная $F$\Hyph компонента линейного отображения $f$}%
   {standard component of linear map, division ring}%
\Index%458%С%стандартная компонента дифференциала Гато отображения f
   {стандартная компонента дифференциала Гато отображения $f$}%
   {standard component of Gateaux differential, division ring}%
\Index%459%С%стандартная компонента квадратичного отображения f над полем F
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения f тела
   {стандартная компонента полилинейного отображения $f$ тела}%
   {standard component of polylinear map, division ring}%
\Index%630%С%стандартная компонента производной Гато отображения f
   {стандартная компонента производной Гато отображения $f$}%
   {standard component of Gateaux derivative, algebra}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor, division ring}%
\Index%574%С%стандартная компонента тензора в тензорном произведении алгебр
   {стандартная компонента тензора в тензорном произведении алгебр}%
   {standard component of tensor, algebra}%
\Index%464%С%стандартное F- представление линейного отображения тела
   {стандартное $F$\Hyph представление линейного отображения тела}%
   {linear map, standard representation, division ring}%
\Index%465%С%стандартное представление дифференциала Гато отображения тела над полем F
   {стандартное представление дифференциала Гато отображения тела над полем $F$}%
   {Gateaux differential, standard representation, division ring}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения тела
   {стандартное представление полилинейного отображения тела}%
   {polylinear map, standard representation, division ring}%
\Index%631%С%стандартное представление производной Гато отображения над алгеброй
   {стандартное представление производной Гато отображения над алгеброй}%
   {Gateaux derivative, standard representation, algebra}%
\Index%471%С%стандартные координаты rcd базиса
   {стандартные координаты \rcd базиса}%
   {standard coordinates of rcd basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%618%С%структурные константы алгебры над кольцом
   {структурные константы алгебры $A$ над кольцом $R$}%
   {structural constants of algebra}%
\Index%473%С%структурные константы тела D над полем F
   {структурные константы тела $D$ над полем $F$}%
   {structural constants of division ring over field}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%475%С%сумма rcd линейных отображений
   {сумма \rcd линейных отображений}%
   {sum of rcd linear maps, rcd vector spaces}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%480%Т%тензорное произведение D- векторных пространств
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Index%481%Т%тензорное произведение Dstar векторных пространств
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Index%573%Т%тензорное произведение алгебр
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Index%482%Т%тензорное произведение колец над коммутативным кольцом
   {тензорное произведение колец над коммутативным кольцом}%
   {tensor product of rings}%
\Index%483%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%484%Т%тензорное произведение тел
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%487%Т%топологическое drc векторное пространство
   {топологическое \drc векторное пространство}%
   {topological drc vector space}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\SetIndexSpace%
\Index%493%У%уравнение Килинга
   {уравнение Килинга}%
   {Killing equation}%
\Index%494%У%уравнение Килинга второго рода
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%500%Ф%фундаментальная последовательность в нормированное теле
   {фундаментальная последовательность в нормированное теле}%
   {fundamental sequence, valued division ring}%
\Index%243%Ф%фундаментальная последовательность в нормированном алгебре
   {фундаментальная последовательность в нормированном алгебре}%
   {fundamental sequence, normed algebra}%
\Index%642%Ф%фундаментальная последовательность в нормированном кольце
   {фундаментальная последовательность в нормированном кольце}%
   {fundamental sequence, normed ring}%
\Index%502%Ф%функция \gi n D- значных переменных
   {функция $\gi n$ $D$\Hyph значных переменных}%
   {function of n D valued variables}%
\Index%501%Ф%функция D- векторного пространства V в D- векторное пространство W, дифференцируемая по Гато
   {функция $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector W$, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, D vector space}%
\Index%625%Ф%функция алгебры, дифференцируемая по Гато
   {функция алгебры, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, algebra}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%505%Ф%функция тела, дифференцируемая по Гато
   {функция тела, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, division ring}%
\Index%506%Ф%функция, непрерывная по совокупности аргументов
   {функция, непрерывная по совокупности аргументов}%
   {function continuous with respect to set of arguments}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $R$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%508%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis, division ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%510%Ч%частная crd производная Гато отображения fb по переменной xa
   {частная \crd производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial crd derivative of map with respect to variable, D vector space}%
\Index%511%Ч%частная drc производная Гато отображения f^b по переменной x^a
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map with respect to variable, D vector space}%
\Index%512%Ч%частная производная Гато отображения f^j по переменной v^i
   {частная производная Гато отображения $f^j$ по переменной $v^i$}%
   {Gateaux partial derivative, D vector space}%
\Index%513%Ч%частное линейное отображение переменной v^i
   {частное линейное отображение переменной $v^i$}%
   {partial linear map of variable}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления F алгебры
   {эндоморфизм представления $\mathfrak{F}$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%324%Э%эффективная башня Tstar- представлений
   {эффективная башня \Ts представлений}%
   {effective tower of representations}%
\Index%516%Э%эффективное Tstar- представление группы
   {эффективное \Ts представление группы}%
   {effective Tstar representation of group}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%517%Э%эффективное представление Omega- алгебры A
   {эффективное представление $\Omega$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $R$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%522%Я%ядро линейного отображения D- векторного пространства
   {ядро линейного отображения $D$\Hyph векторного пространства}%
   {kernel of linear map, D vector space}%
\Index%523%Я%ядро линейного отображения тела
   {ядро линейного отображения тела}%
   {kernel of linear map, division ring}%
\Index%524%Я%ядро неэффективности Tstar- представления группы G
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of Tstar representation of group}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%

\CloseIndex


==> Linear.Mapping.Russian.tex <==
%auto-ignore
\input{Linear.Mapping}

\ifx\PrintBook\undefined
\else
\chapter{Линейное отображение алгебры}
\fi

\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOff
\section{Модуль}

\begin{theorem}
\label{theorem: effective representation of the ring}
Пусть кольцо $D$ имеет единицу $e$.
Представление
\ShowEq{representation of the ring}
кольца $D$
в абелевой группе $A$
\AddIndex{эффективно}{effective representation of ring}
тогда и только тогда, когда
из равенства $f(a)=0$ следует $a=0$.
\end{theorem}
\begin{proof}
Сумма преобразований $f$ и $g$ абелевой группы определяется согласно
правилу
\ShowEq{sum of transformations of Abelian group}
Поэтому, рассматривая представление кольца $D$ в
абелевой группе $A$, мы полагаем
\ShowEq{sum of transformations of Abelian group, 1}
Произведение преобразований представления определено
согласно правилу
\ShowEq{product of transformations of representation}

Если $a$, $b\in R$
порождают одно и то же преобразование, то
\ShowEq{representation of ring, 1}
для любого $m\in A$.
Из равенства
\EqRef{representation of ring, 1}
следует, что $a-b$ порождает нулевое преобразование
\ShowEq{representation of ring, 2}
Элемент $e+a-b$ порождает тождественное преобразование.
Следовательно, представление $f$ эффективно тогда и только тогда,
когда $a=b$.
\end{proof}

\begin{definition}
\label{definition: module over ring}
Пусть $D$ - коммутативное кольцо.
$A$ - \AddIndex{модуль над кольцом}{module over ring} $D$,
если $A$ - абелева группа и
определено эффективное представление кольца $D$
в абелевой группе $A$.
\qed
\end{definition}

\begin{definition}
\label{definition: free module over ring}
$A$ - \AddIndex{свободный модуль над кольцом}{free module over ring} $D$,
если $A$ имеет базис
над кольцом $D$.\footnote{Я следую
определению в \citeBib{Serge Lang}, c. 103.}
\qed
\end{definition}

Следующее определение является следствием определений
\ref{definition: module over ring}
и \xRef{0912.3315}{definition: morphism of representations of F algebra}.

\begin{definition}
\label{definition: linear map from A1 R1 to A2 R2}
Пусть $A_1$ - модуль над кольцом $R_1$.
Пусть $A_2$ - модуль над кольцом $R_2$.
Морфизм
\ShowEq{linear map from A1 R1 to A2 R2}
представления кольца $R_1$ в абелевой группе $A_1$
в представление кольца $R_2$ в абелевой группе $A_2$
называется
\AddIndex{линейным отображением $R_1$\Hyph модуля $A_1$
в $R_2$\Hyph модуль $A_2$}
{linear mapping of R_1 module into R_2 module}.
\qed
\end{definition}

\begin{theorem}
Линейное отображение
\ShowEq{linear map from A1 R1 to A2 R2}
$R_1$\Hyph модуля $A_1$
в $R_2$\Hyph модуль $A_2$
удовлетворяет равенствам\footnote{Предлагаемые равенства в
классической записи имеют вполне знакомый вид
\ShowEq{linear map from A1 R1 to A2 R2, 1, old}}
\ShowEq{linear map from A1 R1 to A2 R2, 1}
\end{theorem}
\begin{proof}
Из определений
\ref{definition: linear map from A1 R1 to A2 R2}
и \xRef{0912.3315}{definition: morphism of representations of F algebra}
следует, что
\begin{itemize}
\item отображение $f$ является гомоморфизмом кольца $R_1$
в кольцо $R_2$ (равенство
\EqRef{linear map from A1 R1 to A2 R2, 1 3})
\item отображение $g$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\EqRef{linear map from A1 R1 to A2 R2, 1 1})
\end{itemize}
Равенство
\EqRef{linear map from A1 R1 to A2 R2, 1 2}
следует из равенства
\xEqRef{0912.3315}
{eq: morphism of representations of F algebra, definition, 2}.
\end{proof}

Согласно теореме
\xRef{0912.3315}{theorem: morphism of representations of algebra, reduce}
при изучении линейных отображений, не нарушая общности,
мы можем полагать $R_1=R_2$.

\begin{definition}
\label{definition: linear map from A1 to A2, module}
Пусть $A_1$ и
$A_2$ - модули над кольцом $D$.
Морфизм
\ShowEq{linear map from A1 to A2}
представления кольца $D$ в абелевой группе $A_1$
в представление кольца $D$ в абелевой группе $A_2$
называется
\AddIndex{линейным отображением $D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$}
{linear mapping of R modules}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: linear map from A1 to A2}
Линейное отображение
\ShowEq{linear map from A1 to A2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
удовлетворяет равенствам\footnote{В классической записи
приведенные равенства имеют вид
\ShowEq{linear map from A1 to A2, 1 old}
}
\ShowEq{linear map from A1 to A2, 1}
\end{theorem}
\begin{proof}
Из определения
\ref{definition: linear map from A1 to A2, module}
и теоремы
\xRef{0912.3315}{theorem: morphism of representations of algebra, reduce}
следует, что
отображение $g$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\EqRef{linear map from A1 to A2, 1 1})
Равенство
\EqRef{linear map from A1 to A2, 1 2}
следует из равенства
\xEqRef{0912.3315}{eq: morphism of representations of F algebra}.
\end{proof}

\section{Алгебра над кольцом}
\label{section: Algebra over Ring}

\else
\newpage
\fi
\begin{definition}
\label{definition: algebra over ring}
Пусть $D$ - коммутативное кольцо.
\ePrints{1003.1544}
\ifx\Semafor\ValueOn
Пусть $A$ - модуль над кольцом $D$.\footnote{Существует
несколько эквивалентных определений алгебры.
Вначале я хотел рассмотреть представление кольца $D$
в абелевой группе кольца $A$.
Однако мне надо было объяснить почему произведение
элементов кольца $D$ и алгебры $A$ коммутативно.
Это потребовало определение центра алгебры $A$.
После тщательного анализа
я выбрал определение, приведенное в
\citeBib{Richard D. Schafer}, с. 1,
\citeBib{0105.155}, с. 4.
%Эта точка зрения имеет ещё два преимущества.
%Во-первых, как следует из теоремы
%если алгебра не имеет единицы, то не существует
%изоморфного образа кольца $D$ в алгебре $A$.
%Во-вторых, я не исключаю возможность рассматривать
%векторное пространство над алгеброй как алгебру.
}
\else
Пусть $A$ - модуль над кольцом $D$.
\fi
Для заданного билинейного отображения
\ShowEq{product in algebra, definition 1}
мы определим произведение в $A$
\ShowEq{product in algebra, definition 2}
$A$ - \AddIndex{алгебра над кольцом}{algebra over ring} $D$,
если $A$ - $D$\Hyph модуль и в $A$
определена операция произведения
\EqRef{product in algebra, definition 2}.
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOff
Алгебра
\ShowEq{opposite algebra}
называется
\AddIndex{алгеброй, противоположной алгебре $A$}{opposite algebra},
если в модуле $A$ определено произведение согласно
правилу\footnote{Определение дано по аналогии
с определением \citeBib{Bourbaki: Algebra 1}-2, с. 19.}
\ShowEq{opposite algebra, product}
\fi
Если $A$ является свободным
$D$\Hyph модулем, то $A$ называется
\AddIndex{свободной алгеброй над кольцом}{free algebra over ring} $D$.
\qed
\end{definition}

\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOff
\begin{remark}
\label{remark: opposite algebra}
Алгебра $A$ и противоположная ей алгебра совпадают как
модули.
\qed
\end{remark}

\begin{theorem}
Произведение в алгебре $A$ дистрибутивно по отношению к сложению.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочки равенств
\ShowEq{product distributive in algebra}
\end{proof}

Произведение в алгебре может быть ни коммутативным,
ни ассоциативным. Следующие определения основаны на
определениях, данным в \citeBib{Richard D. Schafer}, с. 13.

\begin{definition}
\AddIndex{Коммутатор}{commutator of algebra}
\ShowEq{commutator of algebra}
служит мерой коммутативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{коммутативной}{commutative D algebra},
если
\ShowEq{commutative D algebra}
\qed
\end{definition}

\begin{definition}
\AddIndex{Ассоциатор}{associator of algebra}
\ShowEq{associator of algebra}
служит мерой ассоциативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной}{associative D algebra},
если
\ShowEq{associative D algebra}
\qed
\end{definition}

\begin{theorem}
Пусть $A$ - алгебра над коммутативным кольцом $D$.\footnote{Утверждение
теоремы опирается на равенство
\citeBib{Richard D. Schafer}-(2.4).}
\ShowEq{associator of algebra, 1}
для любых $a$, $b$, $c$, $d\in A$.
\end{theorem}
\begin{proof}
Равенство \EqRef{associator of algebra, 1}
следует из цепочки равенств
\ShowEq{associator of algebra, 2}
\end{proof}

\begin{definition}
\AddIndex{Ядро $D$\Hyph алгебры $A$}{nucleus of algebra}
- это множество\footnote{Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 13}
\ShowEq{nucleus of algebra}
\qed
\end{definition}

\begin{definition}
\AddIndex{Центр $D$\Hyph алгебры $A$}{center of algebra}
- это множество\footnote{Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 14}
\ShowEq{center of algebra}
\qed
\end{definition}

\begin{theorem}
\label{theorem: unit of algebra and ring}
Пусть $D$ - коммутативное кольцо.
Если $D$\Hyph алгебра $A$ имеет единицу, то существует
изоморфизм $f$ кольца $D$ в центр алгебры $A$.
\end{theorem}
\begin{proof}
Пусть $e\in A$ - единица алгебры $A$.
Положим $f\circ a=ae$.
\end{proof}
\else
\newpage
\fi

Пусть $\Basis e$ - базис свободной алгебры $A$ над кольцом $D$.
Если алгебра $A$ имеет единицу,
положим $\Vector e_{\gi 0}$ - единица алгебры $A$.

\begin{theorem}
Пусть $\Basis e$ - базис свободной алгебры $A$ над кольцом $D$.
Пусть
\ShowEq{a b in basis of algebra}
Произведение $a$, $b$ можно получить согласно правилу
\ShowEq{product in algebra}
где
\ShowEq{structural constants of algebra}
- \AddIndex{структурные константы алгебры $A$ над кольцом $D$}
{structural constants of algebra}.
Произведение базисных векторов в алгебре $A$ определено согласно правилу
\ShowEq{product of basis vectors, algebra}
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Равенство
\EqRef{product of basis vectors, algebra}
является следствием утверждения, что $\Basis e$
является базисом алгебры $A$.
Так как произведение в алгебре является билинейным отображением,
то произведение $a$ и $b$ можно записать в виде
\ShowEq{product in algebra, 1}
Из равенств
\EqRef{product of basis vectors, algebra},
\EqRef{product in algebra, 1},
следует
\ShowEq{product in algebra, 2}
Так как $\Basis e$ является базисом алгебры $A$, то равенство
\EqRef{product in algebra}
следует из равенства
\EqRef{product in algebra, 2}.
\end{proof}

\begin{theorem}
Если алгебра $A$ коммутативна, то
\ShowEq{commutative product in algebra, 1}
Если алгебра $A$ ассоциативна, то
\ShowEq{associative product in algebra, 1}
\end{theorem}
\begin{proof}
Для коммутативной алгебры,
равенство
\EqRef{commutative product in algebra, 1}
следует из равенства
\ShowEq{commutative product in algebra}
Для ассоциативной алгебры,
равенство
\EqRef{associative product in algebra, 1}
следует из равенства
\ShowEq{associative product in algebra}
\end{proof}
\fi

\section{Линейное отображение алгебры}

\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOff
Алгебра является кольцом. Отображение, сохраняющее
структуру алгебры как кольца, называется гомоморфизмом
алгебры. Однако для нас важнее утверждение, что алгебра
является модулем над коммутативным кольцом.
Отображение, сохраняющее
структуру алгебры как модуля, называется линейным отображением
алгебры.
Таким образом,
следующее определение
опирается на определение
\ref{definition: linear map from A1 to A2, module}.
\fi

\begin{definition}
\label{definition: linear map from A1 to A2, algebra}
Пусть $A_1$ и
$A_2$ - алгебры над кольцом $D$.
Морфизм
\ShowEq{linear map from A1 to A2}
представления кольца $D$ в абелевой группе $A_1$
в представление кольца $D$ в абелевой группе $A_2$
называется
\AddIndex{линейным отображением $D$\Hyph алгебры $A_1$
в $D$\Hyph алгебру $A_2$}
{linear mapping of R algebras}.
Обозначим
\ShowEq{set linear mappings, algebra}
множество линейных отображений
алгебры
$A_1$
в алгебру
$A_2$.
\qed
\end{definition}
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\newpage
\fi

\begin{theorem}
Линейное отображение
\ShowEq{linear map from A1 to A2}
$D$\Hyph алгебры $A_1$
в $D$\Hyph алгебру $A_2$
удовлетворяет равенствам
\ShowEq{linear map from A1 to A2, algebra}
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\else
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: linear map from A1 to A2}.
\end{proof}

\begin{theorem}
\label{theorem: sum of linear maps, algebra}
Рассмотрим алгебру $A_1$ и алгебру $A_2$.
Пусть отображения
\ShowEq{sum of linear maps, algebra}
являются линейными отображениями.
Тогда отображение $f+g$,
определённое равенством
\ShowEq{sum of linear maps, 0, algebra}
также является линейным.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{sum of linear maps, 1, algebra}
\end{proof}

\begin{theorem}
\label{theorem: linear map times constant, algebra}
Рассмотрим алгебру $A_1$ и алгебру $A_2$.
Пусть отображение
\ShowEq{linear map from A1 to A2}
является линейным отображением.
Тогда отображения
\ShowEq{linear map times constant, algebra}
определённые равенствами
\ShowEq{linear map times constant, 0, algebra}
также являются линейными.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{linear map times constant, 1, algebra}
\end{proof}

\begin{theorem}
\label{theorem: linear map times scalar, algebra}
Рассмотрим алгебру $A_1$ и алгебру $A_2$.
Пусть отображение
\ShowEq{linear map from A1 to A2}
является линейным отображением.
Тогда отображения
\ShowEq{linear map times scalar, algebra}
определённое равенством
\ShowEq{linear map times scalar, 0, algebra}
также являются линейными.
При этом выполняется равенство
\ShowEq{linear map times scalar, pq, algebra}
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{linear map times scalar, 1, algebra}
\end{proof}
\fi
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\newpage
\fi

\begin{theorem}
\label{theorem: module of linear mappings}
Пусть $D$ - коммутативное кольцо с единицей.
Рассмотрим $D$\Hyph алгебру $A_1$ и $D$\Hyph алгебру $A_2$.
Множество $\mathcal L(A_1;A_2)$
является $D$\Hyph модулем.
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Теорема \ref{theorem: sum of linear maps, algebra}
определяет сумму линейных отображений из $D$\Hyph алгебры $A_1$
в $D$\Hyph алгебру $A_2$.
Пусть
\ShowEq{module of linear mappings, 1}
Для любого
\ShowEq{module of linear mappings, 2}
Следовательно, сумма линейных отображений коммутативна и ассоциативна.

Отображение $z$, определённое равенством
\ShowEq{module of linear mappings, 3}
является нулём операции сложения, так как
\ShowEq{module of linear mappings, 4}
Для заданного отображения $f$ отображение $g$,
определённое равенством
\ShowEq{module of linear mappings, 5}
удовлетворяет равенству
\ShowEq{module of linear mappings, 6}
так как
\ShowEq{module of linear mappings, 7}
Следовательно, множество $\mathcal L(A_1;A_2)$
является абелевой группой.

Из теоремы
\ref{theorem: linear map times scalar, algebra}
следует, что определенно представление
кольца $D$ в абелевой группе $\mathcal L(A_1;A_2)$.
Так как кольцо $D$ имеет единицу, то согласно теореме
\ref{theorem: effective representation of the ring}
указанное представление эффективно.
\end{proof}

\section{Алгебра \texorpdfstring{$\mathcal L(A;A)$}{L(A;A)}}

\begin{theorem}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Пусть $f$ - линейное отображение из алгебры $A$ в алгебру $B$.
Пусть $g$ - линейное отображение из алгебры $B$ в алгебру $C$.
Отображение $g\circ f$, определённое диаграммой
\ShowEq{product of linear mapping, algebra}
является линейным отображением из алгебры $A$ в алгебру $C$.
\end{theorem}
\begin{proof}
Доказательство теоремы следует из цепочек равенств
\ShowEq{product of linear mapping, algebra, 1}
\end{proof}

\begin{theorem}
\label{theorem: product of linear mapping, algebra, f}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Пусть $f$ - линейное отображение из алгебры $A$ в алгебру $B$.
Отображение $f$ порождает линейное отображение
\ShowEq{product of linear mapping, algebra, f}
\end{theorem}
\begin{proof}
Доказательство теоремы следует из цепочек равенств
\ShowEq{product of linear mapping, algebra, f1}
\end{proof}

\begin{theorem}
\label{theorem: product of linear mapping, algebra, g}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Пусть $g$ - линейное отображение из алгебры $B$ в алгебру $C$.
Отображение $g$ порождает линейное отображение
\ShowEq{product of linear mapping, algebra, g}
\end{theorem}
\begin{proof}
Доказательство теоремы следует из цепочек равенств
\ShowEq{product of linear mapping, algebra, g1}
\end{proof}

\begin{theorem}
\label{theorem: product of linear mapping, algebra, gf}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Отображение
\ShowEq{product of linear mapping, algebra, gf}
является билинейным отображением.
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\ref{theorem: product of linear mapping, algebra, f},
\ref{theorem: product of linear mapping, algebra, g}.
\end{proof}
\fi

\begin{theorem}
\label{theorem: module L(A;A) is algebra}
Пусть $A$ - алгебра над коммутативным кольцом $D$.
Модуль $\mathcal L(A;A)$, оснащённый произведением
\ShowEq{module L(A;A) is algebra}
является алгеброй над $D$.
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\else
\end{theorem}
\begin{proof}
Теорема является следствием определения
\ref{definition: algebra over ring}
и теоремы
\ref{theorem: product of linear mapping, algebra, gf}.
\end{proof}
\fi

\input{Tensor.Algebra.Russian}

\section{Линейное отображение в ассоциативную алгебру}

\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOff
\begin{theorem}
\label{theorem: bilinear mapping A LA}
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения $f\in\mathcal L(A_1;A_2)$
отображение
\ShowEq{bilinear mapping A LA}
является билинейным отображением.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{bilinear mapping A LA, 1}
\end{proof}

\begin{theorem}
\label{theorem: linear map AA LAA}
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения $f\in\mathcal L(A_1;A_2)$
существует линейное отображение
\ShowEq{linear map AA LAA}
определённое равенством
\ShowEq{linear map AA LAA, 1}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теорем
\ref{theorem: tensor product and polylinear mapping},
\ref{theorem: bilinear mapping A LA}.
\end{proof}

\begin{theorem}
\label{theorem: representation module A2 in LA}
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Линейное отображение
\ShowEq{representation A2 in LA}
определённое равенством
\ShowEq{representation A2 in LA, 1}
является представлением\footnote{Определение представления
$\Omega$\Hyph алгебры дано в определении
\xRef{0912.3315}{definition: Tstar representation of algebra}.}
модуля $\ATwo$
в модуле $\mathcal L(A_1;A_2)$.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: linear map times constant, algebra},
отображение \EqRef{representation A2 in LA, 1}
является преобразованием модуля $\mathcal L(A_1;A_2)$.
Для данного тензора $c\in \ATwo$
преобразование $h(c)$ является линейным преобразованием
модуля $\mathcal L(A_1;A_2)$, так как
\ShowEq{representation A2 in LA, 2}
Согласно теореме
\ref{theorem: linear map AA LAA},
отображение \EqRef{representation A2 in LA, 1}
является линейным отображением.
Согласно определению
\xRef{0912.3315}{definition: Tstar representation of algebra}
отображение \EqRef{representation A2 in LA, 1}
является представлением модуля $\ATwo$
в модуле $\mathcal L(A_1;A_2)$.
\end{proof}

\begin{theorem}
\label{theorem: representation algebra A2 in LA}
Пусть $A$ - алгебра над коммутативным кольцом $D$.
Алгебра $A\otimes A$, в которой произведение определено
согласно правилу
\ShowEq{product in algebra AA}
порождает
% эффективное
 представление
в модуле $\mathcal L(A;A)$.
Это представление позволяет отождествить тензор
$d\in A\otimes A$ с преобразованием $d\circ\delta$, где $\delta$ -
тождественное преобразование.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: linear map AA LAA},
отображение $f\in\mathcal L(A;A)$ и тензор $d\in A\otimes A$
порождают отображение
\ShowEq{tensor and mapping in A, algebra}
Если мы положим $f=\delta$, $d=a\otimes b$,
то равенство \EqRef{tensor and mapping in A, algebra}
приобретает вид
\ShowEq{tensor and mapping in A, 1, algebra}
Если мы положим
\ShowEq{tensor and mapping in A, 2, algebra}
то сравнение равенств
\EqRef{tensor and mapping in A, 1, algebra} и
\EqRef{tensor and mapping in A, 2, algebra}
даёт основание отождествить действие тензора
$a\otimes b$ с
преобразованием $(a\otimes b)\circ\delta$.
Следовательно, отображение
\ShowEq{tensor and mapping in A, 3, algebra}
является гомоморфизмом модуля $A\otimes A$ в модуль $\mathcal L(A;A)$.

Отображение \EqRef{tensor and mapping in A, 3, algebra}
является также гомоморфизмом алгебр,
так как произведение преобразований $a\otimes b$ и $c\otimes d$
имеет вид
\ShowEq{tensor and mapping in A, product, algebra}
\end{proof}

Из теоремы \ref{theorem: representation algebra A2 in LA}
следует, что отображение
\EqRef{representation A2 in LA, 1}
можно рассматривать как произведение отображений
$a\otimes b$ и $f$.
Это позволяет вместо представления модуля
$\ATwo$ в модуле $\mathcal L(A_1;A_2)$
рассматривать представление алгебры
$\ATwo$ в модуле $\mathcal L(A_1;A_2)$.

Тензор $a\in \ATwo$
\AddIndex{невырожден}{nonsingular tensor, algebra},
если существует
тензор $b\in \ATwo$ такой, что $a\circ b=1\otimes 1$.

\begin{definition}
Рассмотрим представление алгебры $\ATwo$
в модуле $\mathcal L(A_1;A_2)$.\footnote{Определение дано по
аналогии с определением
\xRef{0912.3315}{definition: orbit of Tstar representation of group}.}
\AddIndex{Орбитой линейного отображения}
{orbit of linear mapping}
$f\in\mathcal L(A_1;A_2)$
называется множество
\ShowEq{orbit of linear mapping}
\qed
\end{definition}
\fi

\begin{theorem}
Рассмотрим $D$\Hyph алгебру $A_1$
и ассоциативную $D$\Hyph алгебру $A_2$.
Рассмотрим представление алгебры $\ATwo$
в модуле $\mathcal L(A_1;A_2)$.
Отображение
\ShowEq{linear map h A1 A2}
порождённое отображением
\ShowEq{linear map f A1 A2}
имеет вид
\ShowEq{h generated by f, associative algebra}
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Произвольный тензор $a\in\ATwo$ можно представить в виде
\ShowEq{h generated by f 1, associative algebra}
Согласно теореме \ref{theorem: representation module A2 in LA},
отображение \EqRef{representation A2 in LA, 1}
линейно.
Это доказывает утверждение теоремы.
\end{proof}

\begin{theorem}
\label{theorem: orbit of linear mapping}
Пусть $A_2$ - алгебра с единицей $e$.
Пусть
\ShowEq{orbit of linear mapping, 02}
- невырожденный тензор.
Орбиты линейных отображений
$f\in\mathcal L(A_1;A_2)$
и \ShowEq{orbit of linear mapping, 01}
совпадают
\ShowEq{orbit of linear mapping, f = g}
\end{theorem}
\begin{proof}
Если
\ShowEq{orbit of linear mapping, 1}
то существует
\ShowEq{orbit of linear mapping, 2}
такое, что
\ShowEq{orbit of linear mapping, 3}
Тогда
\ShowEq{orbit of linear mapping, 4}
Следовательно,
\ShowEq{orbit of linear mapping, 5}
\ShowEq{orbit of linear mapping, g in f}

Так как $a$ - невырожденный тензор, то
\ShowEq{orbit of linear mapping, 6}
Если
\ShowEq{orbit of linear mapping, 5}
то существует
\ShowEq{orbit of linear mapping, 2}
такое, что
\ShowEq{orbit of linear mapping, 7}
Из равенств
\EqRef{orbit of linear mapping, 6},
\EqRef{orbit of linear mapping, 7},
следует, что
\ShowEq{orbit of linear mapping, 8}
Следовательно,
\ShowEq{orbit of linear mapping, 1}
\ShowEq{orbit of linear mapping, f in g}

\EqRef{orbit of linear mapping, f = g}
следует из равенств
\EqRef{orbit of linear mapping, g in f},
\EqRef{orbit of linear mapping, f in g}.
\end{proof}

Из теоремы
\ref{theorem: orbit of linear mapping} также следует, что, если
\ShowEq{orbit of linear mapping, 01}
и \ShowEq{orbit of linear mapping, 02}
- вырожденный тензор, то
отношение
\EqRef{orbit of linear mapping, g in f} верно.
Однако основной результат теоремы
\ref{theorem: orbit of linear mapping}
состоит в том, что представления алгебры
$\ATwo$ в модуле $\mathcal L(A_1;A_2)$
порождает отношение эквивалентности в модуле $\mathcal L(A_1;A_2)$.
Если удачно выбрать представители каждого класса эквивалентности,
то полученное множество будет множеством образующих
рассматриваемого представления.\footnote{Множество образующих
представления определено в определении
\xRef{0912.3315}{definition: generating set of representation}.}

\section{Линейное отображение в свободную
конечно мерную ассоциативную алгебру}
\fi

\begin{theorem}
Пусть $A_1$ - алгебра
над кольцом $D$.
Пусть $A_2$ - свободная конечно мерная ассоциативная алгебра
над кольцом $D$.
Пусть $\Basis e$ - базис алгебры $A_2$ над кольцом $D$.
Отображение
\ShowEq{standard representation of mapping A1 A2, 1, associative algebra}
порождённое отображением $f\in\mathcal(A_1;A_2)$
посредством тензора $a\in\ATwo$, имеет стандартное представление
\ShowEq{standard representation of mapping A1 A2, 2, associative algebra}
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: standard component of tensor, division ring},
стандартное представление тензора $a$ имеет вид
\ShowEq{standard representation of mapping A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of mapping A1 A2, 2, associative algebra}
следует из равенств
\EqRef{standard representation of mapping A1 A2, 1, associative algebra},
\EqRef{standard representation of mapping A1 A2, 3, associative algebra}.
\end{proof}
\fi

\begin{theorem}
\label{theorem: coordinates of mapping A1 A2, algebra}
Пусть $\Basis e_1$ - базис свободной конечно мерной
$D$\Hyph алгебры $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть $B_{2\cdot}{}_{\gi{kl}}^{\gi p}$ - структурные константы алгебры $A_2$.
Координаты отображения
\ShowEq{coordinates of mapping A1 A2, 1}
порождённого отображением $f\in\mathcal(A_1;A_2)$
посредством тензора $a\in\ATwo$, и его стандартные компоненты
связаны равенством
\ShowEq{coordinates of mapping A1 A2, 2, associative algebra}
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Относительно базисов
$\Basis e_1$ и $\Basis e_2$, линейные отображения $f$ и $g$ имеют вид
\ShowEq{coordinates of mappings f g, associative algebra}
Из равенств
\EqRef{coordinates of mapping f, associative algebra},
\EqRef{coordinates of mapping g, associative algebra},
\EqRef{standard representation of mapping A1 A2, 2, associative algebra}
следует
\ShowEq{coordinates of mapping A1 A2, 3, associative algebra}
Так как векторы $\Vector e_{2\cdot\gi k}$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\EqRef{coordinates of mapping A1 A2, 2, associative algebra}
следует из равенства
\EqRef{coordinates of mapping A1 A2, 3, associative algebra}.
\end{proof}

\begin{theorem}
\label{theorem: linear map over ring, matrix}
Пусть $\Basis e_1$ - базис свободной конечно мерной
$D$\Hyph алгебры $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть $B_{2\cdot}{}_{\gi{kl}}^{\gi p}$ - структурные константы алгебры $A_2$.
Рассмотрим матрицу
\ShowEq{linear map over ring, matrix}
строки которой пронумерованы индексом
\ShowEq{linear map over ring, row of matrix}
и столбцы пронумерованы индексом
\ShowEq{linear map over ring, column of matrix}.
Если
матрица $\mathcal B$ невырождена,
то для заданных координат линейного преобразования
\ShowEq{linear map over ring, left side}
и для отображения
\ShowEq{linear map over ring, f=1},
система линейных уравнений
\EqRef{coordinates of mapping A1 A2, 2, associative algebra}
относительно стандартных компонент этого преобразования
$g^{\gi{kr}}$ имеет единственное
решение.

Если
матрица $\mathcal B$ вырождена,
то условием существования решения
системы линейных уравнений
\EqRef{coordinates of mapping A1 A2, 2, associative algebra}
является равенство
\ShowEq{linear map over ring, determinant=0, 1}
В этом случае система линейных уравнений
\EqRef{coordinates of mapping A1 A2, 2, associative algebra}
имеет бесконечно много решений и существует линейная
зависимость между величинами $g_{\gi m}^{\gi k}$.
\end{theorem}
\begin{proof}
Утверждение теоремы
является следствием
теории линейных уравнений над кольцом.
\end{proof}

\begin{theorem}
\label{theorem: linear map over ring, determinant=0}
Пусть $A$ - свободная конечно мерная ассоциативная алгебра
над кольцом $D$.
Пусть $\Basis e$ - базис алгебры $A$ над кольцом $D$.
Пусть $B_{\gi{kl}}^{\gi p}$
- структурные константы алгебры $A$.
Пусть матрица \EqRef{linear map over ring, matrix} вырождена.
Пусть линейное отображение $f\in\mathcal L(A;A)$ невырождено.
Если координаты линейных преобразований $f$ и $g$
удовлетворяют равенству
\ShowEq{linear map over ring, determinant=0, 2}
то система линейных уравнений
\ShowEq{coordinates of mapping A}
имеет бесконечно много решений.
\end{theorem}
\begin{proof}
Согласно равенству
\EqRef{linear map over ring, determinant=0, 2}
и теореме
\ref{theorem: linear map over ring, matrix},
система линейных уравнений
\ShowEq{coordinates of mapping A1 A2, 4f}
имеет бесконечно много решений,
соответствующих линейному отображению
\ShowEq{coordinates of mapping A1 A2, 5f}
Согласно равенству
\EqRef{linear map over ring, determinant=0, 2}
и теореме
\ref{theorem: linear map over ring, matrix},
система линейных уравнений
\ShowEq{coordinates of mapping A1 A2, 4g}
имеет бесконечно много решений,
соответствующих линейному отображению
\ShowEq{coordinates of mapping A1 A2, 5g}
Отображения $f$ и $g$ порождены отображением $\delta$.
Согласно теореме
\ref{theorem: orbit of linear mapping},
отображение $f$ порождает отображение $g$.
Это доказывает утверждение теоремы.
\end{proof}

\begin{theorem}
\label{theorem: linear mapping in L(A,A), associative algebra}
Пусть $A$ - свободная конечно мерная ассоциативная алгебра
над кольцом $D$.
Представление алгебры $A\otimes A$ в алгебре $\mathcal L(A;A)$ имеет
конечный базис $\Basis I$.
\begin{enumerate}
\item \label{f in L(A,A), 1, associative algebra}
Линейное отображение
\ShowEq{f in L(A,A)}
имеет вид
\ShowEq{f in L(A,A), 1, associative algebra}
\item \label{f in L(A,A), 2, associative algebra}
Его стандартное представление имеет вид
\ShowEq{f in L(A,A), 2, associative algebra}
\end{enumerate}
\end{theorem}
\begin{proof}
Из теоремы \ref{theorem: linear map over ring, determinant=0}
следует, что если матрица $\mathcal B$ вырождена
и отображение $f$ удовлетворяет равенству
\ShowEq{linear map over ring, determinant=0, 3}
то отображение $f$ порождает то же самое множество отображений,
что порождено отображением $\delta$.
Следовательно, для того, чтобы построить базис представления
алгебры $A\otimes A$ в модуле $\mathcal L(A;A)$ мы должны выполнить
следующее построение.

Множество решений системы уравнений
\EqRef{coordinates of mapping A}
порождает свободный подмодуль $\mathcal L$ модуля $\mathcal L(A;A)$.
Мы строим базис $(\Vector h_1, ..., \Vector h_k)$ подмодуля $\mathcal L$.
Затем дополняем этот базис линейно независимыми векторами
$\Vector h_{k+1}$, ..., $\Vector h_m$, которые не принадлежат
подмодулю $\mathcal L$, таким образом, что множество векторов
$\Vector h_1$, ..., $\Vector h_m$
является базисом модуля $\mathcal L(A;A)$.
Множество орбит $(A\otimes A)\circ\delta$,
$(A\otimes A)\circ\Vector h_{k+1}$, ..., $(A\otimes A)\circ\Vector h_m$
порождает модуль $\mathcal L(A;A)$.
Поскольку множество орбит конечно, мы можем выбрать орбиты так, чтобы
они не пересекались. Для каждой орбиты мы можем выбрать
представитель, порождающий эту орбиту.
\end{proof}

\begin{example}
Для поля комплексных чисел алгебра $\mathcal L(C;C)$ имеет базис
\ShowEq{basis L(C,C)}
Для алгебры кватернионов алгебра $\mathcal L(H;H)$ имеет базис
\ShowEq{basis L(H,H)}
\qed
\end{example}
\fi

\section{Линейное отображение в неассоциативную алгебру}

Так как произведение неассоциативно, мы можем предположить,
что действие $a$, $b\in A$ на отображение $f$ может быть
представленно либо в виде $a(fb)$, либо в виде $(af)b$.
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOff
Однако это предположение приводит нас к довольно сложной
структуре линейного отображения.
Чтобы лучше представить насколько сложна структура линейного
отображения, мы начнём с рассмотрения левого и правого сдвигов
в неассоциативной алгебре.

\begin{theorem}
Пусть
\ShowEq{left shift algebra}
отображение левого сдвига.
Тогда
\ShowEq{left shift algebra, 1}
где мы определили линейное отображение
\ShowEq{left shift algebra, 2}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{associator of algebra},
\EqRef{left shift algebra}
следует
\ShowEq{left shift algebra, 3}
Равенство \EqRef{left shift algebra, 1}
следует из равенства \EqRef{left shift algebra, 3}.
\end{proof}
%\ShowEq{left shift algebra, 2a}

\begin{theorem}
Пусть
\ShowEq{right shift algebra}
отображение правого сдвига.
Тогда
\ShowEq{right shift algebra, 1}
где мы определили линейное отображение
\ShowEq{right shift algebra, 2}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{associator of algebra},
\EqRef{right shift algebra}
следует
\ShowEq{right shift algebra, 3}
Равенство \EqRef{right shift algebra, 1}
следует из равенства \EqRef{right shift algebra, 3}.
\end{proof}

Пусть
\ShowEq{f over A}
линейное отображение алгебры $A$.
Согласно теореме \ref{theorem: linear map times constant, algebra},
отображение
\ShowEq{g over A}
также линейное отображение.
Однако неочевидно, можем ли мы записать отображение $g$ в виде
суммы слагаемых вида $(ax)b$ и $a(xb)$.

Если $A$ - свободная конечно мерная алгебра, то мы можем предположить,
что линейное отображение имеет стандартное представление в виде\footnote{Выбор
произволен. Мы можем рассмотреть стандартное представление в виде
\ShowEq{linear map, standard representation, nonassociative algebra, 1}
Тогда равенство
\EqRef{coordinates of mapping A1 A2, 2, nonassociative algebra}
имеет вид
\ShowEq{coordinates of mapping A1 A2, 21, nonassociative algebra}
Я выбрал выражение
\EqRef{linear map, standard representation, nonassociative algebra}
так как порядок сомножителей соответствует порядку, выбранному в теореме
\ref{theorem: linear mapping in L(A,A), associative algebra}.}
\ShowEq{linear map, standard representation, nonassociative algebra}
В этом случае мы можем применить
теорему \ref{theorem: linear mapping in L(A,A), associative algebra}
для отображений в неассоциативную алгебру.
\fi

\begin{theorem}
Пусть $\Basis e_1$ - базис свободной конечно мерной
$D$\Hyph алгебры $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной неассоциативной
$D$\Hyph алгебры $A_2$.
Пусть $B_{2\cdot}{}_{\gi{kl}}^{\gi p}$ - структурные константы алгебры $A_2$.
Пусть отображение
\ShowEq{standard representation of mapping A1 A2, 1, nonassociative algebra}
порождённое отображением $f\in\mathcal(A_1;A_2)$
посредством тензора $a\in\ATwo$, имеет стандартное представление
\ShowEq{standard representation of mapping A1 A2, 2, nonassociative algebra}
Координаты отображения
\EqRef{standard representation of mapping A1 A2, 1, nonassociative algebra}
и его стандартные компоненты
связаны равенством
\ShowEq{coordinates of mapping A1 A2, 2, nonassociative algebra}
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Относительно базисов
$\Basis e_1$ и $\Basis e_2$, линейные отображения $f$ и $g$ имеют вид
\ShowEq{coordinates of mappings f g, nonassociative algebra}
Из равенств
\EqRef{coordinates of mapping f, nonassociative algebra},
\EqRef{coordinates of mapping g, nonassociative algebra},
\EqRef{standard representation of mapping A1 A2, 2, nonassociative algebra}
следует
\ShowEq{coordinates of mapping A1 A2, 3, nonassociative algebra}
Так как векторы $\Vector e_{2\cdot\gi k}$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\EqRef{coordinates of mapping A1 A2, 2, nonassociative algebra}
следует из равенства
\EqRef{coordinates of mapping A1 A2, 3, nonassociative algebra}.
\end{proof}
\fi

\begin{theorem}
\label{theorem: linear mapping in L(A,A), nonassociative algebra}
Пусть $A$ - свободная конечно мерная неассоциативная алгебра
над кольцом $D$.
Представление алгебры $A\otimes A$ в алгебре $\mathcal L(A;A)$ имеет
конечный базис $\Basis I$.
\begin{enumerate}
\item \label{f in L(A,A), 1, nonassociative algebra}
Линейное отображение
\ShowEq{f in L(A,A)}
имеет вид
\ShowEq{f in L(A,A), 1, nonassociative algebra}
\item \label{f in L(A,A), 2, nonassociative algebra}
Его стандартное представление имеет вид
\ShowEq{f in L(A,A), 2, nonassociative algebra}
\end{enumerate}
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Рассмотрим матрицу
\EqRef{linear map over ring, matrix}.
Если
матрица $\mathcal B$ невырождена,
то для заданных координат линейного преобразования
\ShowEq{linear map over ring, left side}
и для отображения
\ShowEq{linear map over ring, f=1},
система линейных уравнений
\EqRef{coordinates of mapping A1 A2, 2, nonassociative algebra}
относительно стандартных компонент этого преобразования
$g^{\gi{kr}}$ имеет единственное
решение.
Если
матрица $\mathcal B$ вырождена,
то согласно теореме
\ref{theorem: linear mapping in L(A,A), associative algebra}
существует конечный базис $\Basis I$,
порождающий множество линейных отображений.
\end{proof}
\fi

В отличие от случая ассоциативной алгебры
множество генераторов $I$ в теореме
\ref{theorem: linear mapping in L(A,A), nonassociative algebra}
не является минимальным.
Из равенства \EqRef{left shift algebra, 1}
следует, что неверно равенство
\EqRef{orbit of linear mapping, 4}.
Следовательно, орбиты отображений
$I_k$ не порождают отношения эквивалентности в алгебре $L(A;A)$.
Так как мы рассматриваем только отображения вида $(aI_k)b$, то
возможно, что при $k\ne l$ отображение $I_k$ порождает отображение $I_l$,
если рассмотреть все возможные операции в алгебре $A$.
Поэтому множество образующих $I_k$ неассоциативной алгебры $A$
не играет такой критической роли как отображение сопряжения в
поле комплексных чисел.
Ответ на вопрос насколько важно отображение $I_k$ в
неассоциативной алгебре требует дополнительного исследования.


==> Mappings.Matrix.Russian.tex <==
%auto-ignore
\input{Mappings.Matrix}
\chapter{Матрица отображений}
\label{chapter: Matrix of Mappings}

\section{Произведение отображений}

На множестве отображений
\ShowEq{set of mappings A}
определено произведение согласно правилу
\ShowEq{set of mappings A, product}
Равенство
\ShowEq{f circ g = g circ f}
справедливо тогда и только тогда, когда диаграма
\ShowEq{f circ g = g circ f, diagram}
коммутативна.

Для $a\in A$, существует отображение
\ShowEq{mapping f a=a}
Если мы будем обозначать отображение $f_a$ буквой $a$,
то опираясь на равенство
\EqRef{set of mappings A, product},
положим
\ShowEq{set of mappings A, product over scalar}

Если $A$ - $\Omega$\Hyph алгебра,
в которой определена операция умножения, то
элемент $a\in A$ так же может служить для обозначения операции
левого сдвига
\ShowEq{set of mappings A, left shift}
Запись \EqRef{set of mappings A, left shift}
не противоречит записи
\EqRef{set of mappings A, product over scalar}.
Однако надо помнить, что произведение
\ShowEq{set of mappings A, nonassociative}
неассоциативно, так как
\ShowEq{set of mappings A, nonassociative, 1}

\section{Бикольцо матриц отображений}

Пусть $A$ - $\Omega$\Hyph алгебра
(\citeBib{Burris Sankappanavar,Cohn: Universal Algebra}),
в которой определена операция сложения.
Мы будем предполагать, что
алгебра $A$ является группой по отношению к
операции сложения.

Пусть
\ShowEq{set of mappings of A}
множество отображений $\Omega$\Hyph алгебры $A$.
Мы можем отобразить операцию сложения в $\Omega$\Hyph алгебре $A$
на множество
\ShowEq{set of mappings of A}
согласно правилу
\ShowEq{set F of mappings A, sum}
Равенство \EqRef{set F of mappings A, sum 1}
является выражением закона дистрибутивности произведения отображений
слева.
Поэтому естественно потребовать, чтобы произведение было дистрибутивно справа
\ShowEq{set F of mappings A, sum 4}
В секции \ref{section: Quasideterminant of Matrix of Mappings}
мы увидим, что это требование существенно.
Следовательно, множество \ShowEq{set of mappings of A}
является множеством гомоморфизмов группы $A$.

Мы требуем, чтобы множество
\ShowEq{set of mappings of A}
было замкнуто относительно операций
сложения и произведения отображений.

\begin{theorem}
Для любого отображения
\ShowEq{set of mappings of A, 2}
справедливы равенства
\ShowEq{set of mappings of A, 3}
\end{theorem}
\begin{proof}
Из равенства
\EqRef{set F of mappings A, sum 3}
следует
\ShowEq{set of mappings of A, 4}
Равенство \EqRef{set of mappings of A, 3 1} следует из равенства
\EqRef{set of mappings of A, 4}.
Из равенства
\EqRef{set F of mappings A, sum 1}
следует
\ShowEq{set of mappings of A, 5}
Равенство \EqRef{set of mappings of A, 3 2} следует из равенства
\EqRef{set of mappings of A, 5}.
\end{proof}

\begin{remark}
Если сумма некоммутативна, то требование замкнутости множества
\ShowEq{set of mappings of A}
относительно операции сложения может оказаться слишком строгим.
Рассмотрим выражение
\ShowEq{noncommutative sum of functions}
Так как, вообще говоря,
\ShowEq{noncommutative sum of functions, 1}
то мы не можем утверждать, что
\ShowEq{noncommutative sum of functions, 2}
В дальнейшем тексте мы будем предполагать, что сложение коммутативно.
Тем не менее все построения в этой главе мы будем выполнять так,
как мы это делали бы в случае некоммутативного сложения.
\qed
\end{remark}

Рассмотрим множество
\AddIndex{матриц отображений}{matrix of mappings},
элементы которых
являются отображениями
\ShowEq{set of mappings of A, 1}.
Согласно определению
\xRef{0701.238}{definition: rc-product of matrices},
мы определим
\AddIndex{$\RCcirc$\Hyph произведение матриц отображений}
{rc product of matrices of mappings}
\ShowEq{rc product of matrices of mappings}
Согласно определению
\xRef{0701.238}{definition: cr-product of matrices},
мы определим
\AddIndex{$\CRcirc$\Hyph произведение матриц отображений}
{cr product of matrices of mappings}
\ShowEq{cr product of matrices of mappings}

\ifx\texFuture\Defined
\begin{definition}
Пусть $A$ - $\Omega$\Hyph алгебра.
Тогда на множестве $A^n$ можно определить структуру
$\Omega$\Hyph алгебры таким образом, что все операции
выполняются покомпонентно. А именно,
если $\omega$ - $p$\Hyph арная операция,
то для заданных кортежей
\ShowEq{Cartesian power of algebra, 1}
действие операции $\omega$ определено согласно правилу
\ShowEq{Cartesian power of algebra, 2}
$\Omega$\Hyph алгебра $A^n$ называется
\AddIndex{декартовой степенью $n$ $\Omega$\Hyph алгебры}
{Cartesian power of algebra} $A$.
\qed
\end{definition}

\begin{definition}
Пусть $A$ - $\Omega$\Hyph алгебра,
в которой определена операция сложения.
Функциональная матрица $a$ называется
\AddIndex{матрицей эндоморфизмов $\Omega$\Hyph алгебры}
{matrix of endomorphisms of H algebra}
$A$, если $a_i^j$ является эндоморфизмом $\Omega$\Hyph алгебры $A$.
\qed
\end{definition}

\begin{theorem}
Пусть $A$ - $\Omega$\Hyph алгебра,
в которой определена операция сложения.
$n\times n$ матрица эндоморфизмов $\Omega$\Hyph алгебры $A$
является эндоморфизмом $\Omega$\Hyph алгебры $A^n$.
\end{theorem}
\begin{proof}
Пусть $f$ - матрица эндоморфизмов $\Omega$\Hyph алгебры $A$.
Тогда для
\ShowEq{matrix of endomorphism, 1}
Если $\omega$ - $p$\Hyph арная операция, то
\ShowEq{matrix of endomorphism, 2}
\end{proof}
\fi

\begin{theorem}
\label{theorem: product of mappings of the set is associative}
Произведение преобразований множества $A$
ассоциативно.\footnote{Утверждение теоремы основано
на примере полугруппы
из \citeBib{Kurosh: General Algebra}, с. 20, 21.}
\end{theorem}
\begin{proof}
Рассмотрим отображения
\ShowEq{mappings of the set}
Утверждение теоремы следует из цепочки равенств
\ShowEq{mappings of the set, 1}
\end{proof}

\begin{theorem}
Множество \ShowEq{set of mappings of A}
является кольцом.
\end{theorem}
\begin{proof}
\ShowEq{set of mappings of A} - абелева группа относительно операции сложения.
Согласно теореме
\ref{theorem: product of mappings of the set is associative},
\ShowEq{set of mappings of A} - полугруппа относительно умножения.
Так как \ShowEq{set of mappings of A, 1} - гомоморфизм абелевой группы $A$,
то для любого $a\in A$
\ShowEq{R(A) distributive, 1}
Из равенства \EqRef{R(A) distributive, 1} следует
закон дистрибутивности
\ShowEq{R(A) distributive, 2}
\end{proof}

Отображения, принадлежащие кольцу \ShowEq{set of mappings of A}, мы также будем называть
\AddIndex{\ShowEq{set of mappings of A}\Hyph отображениями}{A(A) mapping}.

\begin{theorem}
$\RCcirc$\Hyph произведение матриц \ShowEq{set of mappings of A}\Hyph отображений
является матрицей \ShowEq{set of mappings of A}\Hyph отображений.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из уравнения
\EqRef{rc product of matrices of mappings}
и утверждения, что сумма и произведение \ShowEq{set of mappings of A}\Hyph отображений
является \ShowEq{set of mappings of A}\Hyph отображением.
\end{proof}

\begin{theorem}
\label{theorem: product of matrices of mappings is associative}
Произведение матриц \ShowEq{set of mappings of A}\Hyph отображений
ассоциативно.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочки равенств
\ShowEq{product of matrices of mappings is associative}
\end{proof}

\section{Квазидетерминант матрицы отображений}
\label{section: Quasideterminant of Matrix of Mappings}

\begin{theorem}
\label{theorem: rc inverse minor, matrix of mappings}
Предположим, что $n\times n$ матрица
\ShowEq{set of mappings of A}\Hyph отображений $a$
имеет $\RCcirc$\Hyph обратную матрицу\footnote{Это утверждение
и его доказательство основаны
на утверждении 1.2.1 из \citeBib{math.QA-0208146}
(\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=8}{page 8})
для матриц над свободным кольцом с делением.}
\ShowEq{rc inverse matrix of mappings, definition}
Тогда $k\times k$ минор $\RCcirc$\Hyph обратной матрицы
удовлетворяет следующему равенству, при условии, что рассматриваемые
обратные матрицы существуют,
\ShowEq{rc inverse minor, matrix of mappings}
\end{theorem}
\begin{proof}
Определение \EqRef{rc inverse matrix of mappings, definition}
$\RCcirc$\Hyph обратной матрицы
приводит к системе линейных уравнений
\ShowEq{rc inverse minor, matrix of mappings, 1}
Мы умножим \EqRef{rc inverse minor, matrix of mappings, 1, 1} на
\ShowEq{rc inverse minor, matrix of mappings, 3}
Теперь мы можем подставить
\EqRef{rc inverse minor, matrix of mappings,3} в
\EqRef{rc inverse minor, matrix of mappings, 1, 2}
\ShowEq{rc inverse minor, matrix of mappings, 4}
\EqRef{rc inverse minor, matrix of mappings}
следует из \EqRef{rc inverse minor, matrix of mappings, 4}.
\end{proof}

\begin{corollary}
\label{corollary: rc inverse matrix of mappings}
Предположим, что $n\times n$ матрица
\ShowEq{set of mappings of A}\Hyph отображений $a$
имеет $\RCcirc$\Hyph обратную матрицу.
Тогда элементы $\RCcirc$\Hyph обратной матрицы удовлетворяют
равенству
\ShowEq{rc inverse matrix of mappings}
\qed
\end{corollary}

\begin{definition}
\AddIndex{$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}
{j i RCcirc-quasideterminant}
$n\times n$ матрицы $a$
- это формальное выражение
\ShowEq{j i RCcirc-quasideterminant definition}
Согласно замечанию
\xRef{0701.238}{remark: combine the notation of indexes}
мы можем рассматривать $(^b_a)$\hyph $\RCcirc$\Hyph квазидетерминант
как элемент матрицы
\ShowEq{RCcirc-quasideterminant definition},
которую мы будем называть
\AddIndex{$\RCcirc$\Hyph квазидетерминантом}
{RCcirc-quasideterminant definition}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: quasideterminant and inverse, RCcirc}
Выражение для элементов $\RCcirc$\Hyph обратной матрицы имеет вид
\ShowEq{quasideterminant and inverse, RCcirc}
\end{theorem}
\begin{proof}
\EqRef{quasideterminant and inverse, RCcirc} следует
из \EqRef{j i RCcirc-quasideterminant definition}.
\end{proof}

\begin{theorem}
Выражение для
$(^a_b)$\hyph $\RCcirc$\Hyph квазидетерминанта
имеет любую из следующих форм
\ShowEq{RCcirc quasideterminant, expression}
\end{theorem}
\begin{proof}
Утверждение  следует
из \EqRef{rc inverse matrix of mappings} и
\EqRef{j i RCcirc-quasideterminant definition}.
\end{proof}

\begin{definition}
\label{definition: quasideterminant in quasiclosed ring}
Если для отображения \ShowEq{set of mappings of A, 1}
из существования обратного отображения
$f^{-1}$ следует
\ShowEq{set of mappings of A, 6},
то кольцо \ShowEq{set of mappings of A} отображений называется
\AddIndex{квазизамкнутым}{quasiclosed ring of mappings}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: quasideterminant in quasiclosed ring}
Пусть \ShowEq{set of mappings of A} - квазизамкнутое кольцо отображений
$\Omega$\Hyph алгебры $A$.
Пусть $a$ - матрица \ShowEq{set of mappings of A}\Hyph отображений.
Тогда матрицы
$\det\left(a,\RCcirc\right)$ и
$a^{-1\RCcirc}$ являются
матрицами \ShowEq{set of mappings of A}\Hyph отображений.
\end{theorem}
\begin{proof}
Мы докажем теорему индукцией по порядку матрицы.

При $n=1$ из равенства
\EqRef{RCcirc quasideterminant, expression, 1}
следует
\ShowEq{quasideterminant of matrix of linear mappings, 1}
Следовательно, квазидетерминант является матрицей
\ShowEq{set of mappings of A}\Hyph отображений.
Из определения
\ref{definition: quasideterminant in quasiclosed ring}
следует, что матрица $a^{-1\RCcirc}$ является
матрицей \ShowEq{set of mappings of A}\Hyph отображений.

Пусть утверждение теоремы верно для $n-1$.
Пусть $a$ - $n\times n$ матрица.
Согласно предположению индукции, матрица
\ShowEq{minor of RCcirc quasideterminant}
в равенстве
\EqRef{RCcirc quasideterminant, expression, 1}
является матрицей \ShowEq{set of mappings of A}\Hyph отображений.
Следовательно,
$(^a_b)$\hyph $\RCcirc$\Hyph квазидетерминант
является \ShowEq{set of mappings of A}\Hyph отображением.
Из определения
\ref{definition: quasideterminant in quasiclosed ring}
и теоремы
\ref{theorem: quasideterminant and inverse, RCcirc}
следует, что матрица $a^{-1\RCcirc}$ является
матрицей \ShowEq{set of mappings of A}\Hyph отображений.
\end{proof}

\begin{definition}
Если $n\times n$ матрица $a$
\ShowEq{set of mappings of A}\Hyph отображений имеет
$\RCcirc$\Hyph обратную матрицу,
мы будем называть матрицу $a$
\AddIndex{$\RCcirc$\Hyph невырожденной матрицей
\ShowEq{set of mappings of A}\Hyph отображений}
{RCcirc nonsingular matrix of A(A) mappings}.
В противном случае, мы будем называть такую матрицу
\AddIndex{$\RCcirc$\Hyph вырожденной матрицей \ShowEq{set of mappings of A}\Hyph отображений}
{RCcirc singular matrix of A(A) mappings}.
\qed
\end{definition}

\section{Система аддитивных уравнений}

Пусть \ShowEq{set of mappings of A} - квазизамкнутое кольцо отображений
$\Omega$\Hyph алгебры $A$.
Система уравнений
\ShowEq{System of Additive Equations}
где $a$ - матрица \ShowEq{set of mappings of A}\Hyph отображений, называется
\AddIndex{системой аддитивных уравнений}{system of additive equations}.
Систему аддитивных уравнений
\EqRef{System of Additive Equations}
можно записать также в виде
\ShowEq{System of Additive Equations, 1}

\begin{definition}
Предположим, что $a$
- $\RCcirc$\Hyph невырожденная матрица. Мы будем называть
соответствующую систему
аддитивных уравнений
\EqRef{System of Additive Equations}
\AddIndex{$\RCcirc$\Hyph невырожденной системой аддитивных уравнений}
{RCcirc nonsingular system of additive equations}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: nonsingular system of R(A) equations in algebra}
Решение невырожденной системы \ShowEq{set of mappings of A}\Hyph уравнений
\EqRef{System of Additive Equations}
определено однозначно
и может быть записано в любой из следующих форм
\ShowEq{nonsingular system of R(A) equations}
\end{theorem}
\begin{proof}
Умножая обе части равенства
\EqRef{System of Additive Equations}
слева на $a^{-1\RCcirc}$, мы получим
\EqRef{nonsingular system of R(A) equations, solution, matrix}.
Пользуясь определением
\EqRef{j i RCcirc-quasideterminant definition},
мы получим
\EqRef{nonsingular system of R(A) equations, solution, quasideterminant}.
%Решение системы единственно в силу теоремы
%\xEqRef{0612.111}{theorem: two products equal}.
\end{proof}

\begin{example}
Согласно определению
\xRef{0701.238}{definition: Tstar vector space}
эффективное \Ts представление тела $D$
в абелевой группе $\Vector V$
порождает тело отображений $D(*\Vector V)$.
Образ $\Vector v\in\Vector V$
при отображении $a\in D(*\Vector V)$ определён согласно правилу
\ShowEq{mapping D(*V), image}
Произведение отображений $a$, $b\in D(*\Vector V)$
определён согласно правилу
\ShowEq{mapping D(*V), product}
Система аддитивных уравнений в этом случае является системой
\rcd линейных уравнений.
\qed
\end{example}

\begin{example}
Согласно определению
\xRef{0701.238}{definition: Tstar vector space}
эффективное \sT представление тела $D$
в абелевой группе $\Vector V$
порождает тело отображений $D(\Vector V*)$.
Образ $\Vector v\in\Vector V$
при отображении $a\in D(\Vector V*)$ определён согласно правилу
\ShowEq{mapping D(V*), image}
Произведение отображений $a$, $b\in D(\Vector V*)$
определён согласно правилу
\ShowEq{mapping D(V*), product}
Система аддитивных уравнений в этом случае является системой
\dcr линейных уравнений.
\qed
\end{example}

\section{Система аддитивных уравнений в поле комплексных чисел}

Согласно теореме
\xRef{0812.4763}{theorem: real subring of center}
аддитивное отображение поля комплексных чисел линейно
над полем действительных чисел.
Рассмотрим базис
\ShowEq{complex basis over real}
поля комплексных чисел над полем действительных чисел.
В базисе $\Basis e$ аддитивное отображение $f$
определено матрицей
\ShowEq{complex additive map, matrix}
Согласно теореме
\xRef{0812.4763}{theorem: complex field over real field}
линейное отображение имеет матрицу
\ShowEq{complex linear map, matrix}
Это отображение соответствует умножению на число
\ShowEq{complex linear map, matrix 0}
Утверждение следует из равенств
\ShowEq{complex linear map, matrix 1}

Аддитивное отображение, порождённое
отображением сопряжения
\ShowEq{congugate mapping complex field}
имеют матрицу
\ShowEq{congugate mapping complex field, 1}
которая соответствует преобразованию
\ShowEq{congugate mapping complex field, 2}
Утверждение следует из равенств
\ShowEq{congugate mapping complex field, 3}

\begin{theorem}
\label{theorem: additive map of complex field, structure}
Аддитивное отображение поля комплексных чисел имеет вид
\ShowEq{additive map of complex field, structure}
\end{theorem}
\begin{proof}
Пусть отображение $f$ определено матрицей
\EqRef{complex additive map, matrix}.
Сопоставление матриц отображений $f$, $a$, $b$
приводит к матричному равенству
\ShowEq{additive map of complex field, structure, 1}
Из равенств
\EqRef{additive map of complex field, structure 0 0},
\EqRef{additive map of complex field, structure 1 1}
следует
\ShowEq{additive map of complex field, structure, 2}
Из равенств
\EqRef{additive map of complex field, structure 1 0},
\EqRef{additive map of complex field, structure 0 1}
следует
\ShowEq{additive map of complex field, structure, 3}
\end{proof}

В поле комплексных чисел множество аддитивных отображений
порождает кольцо, порождённое операцией умножения на
комплексное число и операцией сопряжения.

\begin{theorem}
Кольцо отображений $\mathcal A(C,C)$ квазизамкнуто.
\end{theorem}
\begin{proof}
Аддитивное отображение невырожденно тогда и только тогда,
когда невырождена его матрица
\EqRef{complex additive map, matrix}.
Обратная матрица также описывает некоторое отображение.
Произведение этих матриц является тождественным преобразованием.
\end{proof}

\begin{theorem}
Произведение аддитивных отображений
\ShowEq{complex additive map f}
\ShowEq{complex additive map g}
имеет вид
\ShowEq{complex additive map fg}
где
\ShowEq{complex additive map h}
\end{theorem}
\begin{proof}
Непосредственной проверкой легко убедиться, что
\ShowEq{complex additive map II=1}
Из цепочки равенств
\ShowEq{complex additive map Ia=bI}
следует
\ShowEq{complex additive map Ia=bI, 1}
Из равенств
\EqRef{complex additive map II=1},
\EqRef{complex additive map Ia=bI, 1}
следует
\ShowEq{complex additive map Ia=bI, 2}
Из равенств
\EqRef{complex additive map II=1},
\EqRef{complex additive map Ia=bI, 2}
следует
\ShowEq{complex additive map h, 1}
Равенство
\EqRef{complex additive map h}
следует из равенства
\EqRef{complex additive map h, 1}.
\end{proof}

\begin{theorem}
\label{theorem: inverse complex additive map}
Пусть аддитивное отображение поля комплексных чисел
\ShowEq{complex additive map g}
является отображением, обратным аддитивному отображению
\ShowEq{complex additive map f}
Тогда
\ShowEq{complex additive map g inverse f}
\end{theorem}
\begin{proof}
Согласно утверждению теоремы
\ShowEq{complex additive map g inverse f, 1}
Из равенств
\EqRef{complex additive map h},
\EqRef{complex additive map g inverse f, 1}
следует
\ShowEq{complex additive map g inverse f, 2}
Из уравнения
\EqRef{complex additive map g inverse f, 2, 2}
следует
\ShowEq{complex additive map g inverse f, 3}
Из уравнений
\EqRef{complex additive map g inverse f, 2, 1},
\EqRef{complex additive map g inverse f, 3}
следует
\ShowEq{complex additive map g inverse f, 4}
\EqRef{complex additive map g inverse f}
следует из равенств
\EqRef{complex additive map g inverse f, 4},
\EqRef{complex additive map g inverse f, 3}.
\end{proof}

\begin{example}
\label{example: system of additive equations, complex field}
Рассмотрим систему аддитивных уравнений
\ShowEq{system of additive equations, complex field}
Систему уравнений
\EqRef{system of additive equations, complex field}
нельзя решать пользуясь определителем и правилом Крамера.
Запишем систему уравнений
\EqRef{system of additive equations, complex field}
в виде
\ShowEq{system of additive equations, complex field, 1}
Найдём $\RCcirc$\Hyph квазидетерминант матрицы
\ShowEq{system of additive equations, complex field, 2}
Согласно равенству
\EqRef{RCcirc quasideterminant, expression, 1}
мы имеем
\ShowEq{system of additive equations, complex field, 3}
Согласно теоремам
\ref{theorem: quasideterminant and inverse, RCcirc},
\ref{theorem: inverse complex additive map},
$\RCcirc$\Hyph обратная матрица имеет вид
\ShowEq{system of additive equations, complex field, 4}
Согласно теореме
\ref{theorem: nonsingular system of R(A) equations in algebra}
решение системы аддитивных уравнений
\EqRef{system of additive equations, complex field}
имеет вид
\ShowEq{system of additive equations, complex field, 5}
Непосредственная проверка показывает, что мы нашли решение системы
уравнений \EqRef{system of additive equations, complex field}
\ShowEq{system of additive equations, complex field, 6}
\qed
\end{example}

\ifx\texFuture\Defined
\section{Пример из алгебры кватернионов}

Чтобы рассмотреть пример $\Omega$\Hyph группы, где операция сложения
некоммутативна, мы изменим набор операций в алгебре кватернионов.
Для того, чтобы обозначения операций не приводило к неоднозначности,
мы введём новые обозначения для операций. 
Сумму мы определим согласно правилу
\ShowEq{quaternion omega group, sum}
Обратный элемент определён операцией
\ShowEq{quaternion omega group, minus}
Мы также определим действие
\ShowEq{quaternion omega group, circ}
Мы положим, что выражение
\ShowEq{quaternion omega group, circ, 1}
эквивалентно выражению
\ShowEq{quaternion omega group, circ, 2}

\begin{theorem}
Рассмотренные операции в $\Omega$\Hyph группе $H$
удовлетворяют равенствам
\ShowEq{quaternion omega group}
\end{theorem}
\begin{proof}
Равенство \EqRef{quaternion omega group, 1}
следует из цепочки равенств
\ShowEq{quaternion omega group, 11}
Равенство \EqRef{quaternion omega group, 2}
следует из цепочки равенств
\ShowEq{quaternion omega group, 21}
Равенство \EqRef{quaternion omega group, 3}
следует из цепочки равенств
\ShowEq{quaternion omega group, 31}
Равенство \EqRef{quaternion omega group, 4}
следует из цепочки равенств
\ShowEq{quaternion omega group, 41}
\end{proof}

\begin{theorem}
Если $a\ne 0$, то отображение $ad(a)$ невырожденно
\ShowEq{quaternion omega group, nonsingular}
\end{theorem}
\begin{proof}
Равенство \EqRef{quaternion omega group, nonsingular}
следует из цепочки равенств
\ShowEq{quaternion omega group, nonsingular, 1}
\end{proof}

\begin{theorem}
Система аддитивных уравнений
\ShowEq{quaternion omega group, additive system}
равносильна системе уравнений
\ShowEq{quaternion omega group, system}
\end{theorem}
\begin{proof}
Подставив равенства
\EqRef{quaternion omega group, sum},
\EqRef{quaternion omega group, circ}
в равенство
\EqRef{quaternion omega group, additive system},
мы получим систему уравнений
\ShowEq{quaternion omega group, additive system, 1}
Положим
\ShowEq{quaternion omega group, system, 1}
\EqRef{quaternion omega group, system}
следует из равенств
\EqRef{quaternion omega group, additive system, 1},
\EqRef{quaternion omega group, system, 1}.
\end{proof}

\begin{remark}
\label{remark: quaternion omega group, system}
Попытка решить систему адитивных уравнений
\EqRef{quaternion omega group, additive system}
- непростая задача, так как
\ShowEq{sum ad, quaternion omega group},
вообще говоря, является многочленом второй степени.
Однако, если $n=2$ система уравнений
\ShowEq{quaternion omega group, system n=2}
может приведена к более простой форме
\ShowEq{quaternion omega group, system n=2, 1}
После замены переменных
\ShowEq{quaternion omega group, system n=2, 2}
система уравнений
\EqRef{quaternion omega group, system n=2, 1}
приобретает вид
\ShowEq{quaternion omega group, system n=2, 3}
Система уравнений
\EqRef{quaternion omega group, system n=2, 3}
эквивалентна системе аддитивных уравнений
\ShowEq{quaternion omega group, additive system n=2}
Найдём $\RCcirc$\Hyph квазидетерминант матрицы
\ShowEq{quaternion omega group, additive system n=2, 1}
Согласно равенству
\EqRef{RCcirc quasideterminant, expression, 1}
мы имеем
\ShowEq{quaternion omega group, additive system n=2, 2}
Согласно теоремам
\ref{theorem: quasideterminant and inverse, RCcirc},
\ref{theorem: inverse complex additive map},
$\RCcirc$\Hyph обратная матрица имеет вид
\ShowEq{quaternion omega group, additive system n=2, 3}
Согласно теореме
\ref{theorem: nonsingular system of R(A) equations in algebra}
решение системы аддитивных уравнений
\EqRef{quaternion omega group, additive system n=2}
имеет вид
\ShowEq{quaternion omega group, additive system n=2, 4}
\qed
\end{remark}

\ShowEq{0 matrix 0}
\ShowEq{0 matrix 1}
\ShowEq{0 matrix 2}

\begin{example}
\label{example: system of additive equations, quaternion}
Мы будем решать систему уравнений
\ShowEq{system of equations, quaternion}
согласно замечанию \ref{remark: quaternion omega group, system}.
После замены переменных
\ShowEq{quaternion omega group, system n=2, 2 1}
система уравнений
\EqRef{system of equations, quaternion}
примет вид
\ShowEq{quaternion omega group, system n=2, 3 1}
где
\ShowEq{quaternion omega group, system n=2, 3 2}
Следовательно, мы можем записать систему уравнений
\EqRef{quaternion omega group, system n=2, 3 1}
в виде системы аддитивных уравнений
\ShowEq{system of additive equations, quaternion, 1}
Найдём $\RCcirc$\Hyph квазидетерминант матрицы
\ShowEq{system of additive equations, quaternion, 2}
Согласно равенству
\EqRef{RCcirc quasideterminant, expression, 1}
мы имеем
\ShowEq{system of additive equations, quaternion, 3}
Согласно теоремам
\ref{theorem: quasideterminant and inverse, RCcirc},
\ref{theorem: inverse complex additive map},
$\RCcirc$\Hyph обратная матрица имеет вид
\ShowEq{system of additive equations, complex field, 4}
Согласно теореме
\ref{theorem: nonsingular system of R(A) equations in algebra}
решение системы аддитивных уравнений
\EqRef{system of additive equations, complex field}
имеет вид
\ShowEq{system of additive equations, complex field, 5}
Непосредственная проверка показывает, что мы нашли решение системы
уравнений \EqRef{system of additive equations, complex field}
\ShowEq{system of additive equations, complex field, 6}
\qed
\end{example}
\fi


==> Octonion.Russian.tex <==
%auto-ignore
\ePrints{1003.1544}
\ifx\Semafor\ValueOff
\chapter{Алгебра октонионов}
\fi

\input{Octonion}

\section{Алгебра октонионов}

\begin{definition}
Алгебра \symb{O}1{octonion algebra} называется
\AddIndex{алгеброй
октонионов}{octonion algebra}%\footnote{Я
%буду следовать определению из \citeBib{0105.155}, с. 6.},
если алгебра имеет базис
\ShowEq{basis of octonion}
и произведение в алгебре $O$ определено согласно правилам
\ShowEq{product in octonion, table}
\qed
\end{definition}

\begin{theorem}
\label{theorem: Octonion Algebra}
Структурные константы алгебры октонионов $O$ относительно базиса
\EqRef{basis of octonion} имеют вид
\ShowEq{structural constants, octonion}
\end{theorem}
\begin{proof}
Значение структурных констант следует из таблицы умножения
\EqRef{product in octonion, table}.
\end{proof}

\section{Линейная функция алгебры октонионов}

Так как вычисления в этом разделе занимают много места,
я собрал в одном месте ссылки на теоремы в этом разделе.
\begin{description}
\item [Теорема \ref{theorem: Standard components of linear function, octonion}]
определение координат линейного отображения
алгебры октонионов $O$
через стандартные компоненты этого отображения.
\item [Равенство \EqRef{octonion, 3, B->A}]
матричная форма зависимости координат линейного отображения
алгебры октонионов $O$
от стандартных компонент этого отображения.
\item [Равенство \EqRef{octonion, 3, A->B}]
матричная форма зависимости стандартных компонент линейного отображения
алгебры октонионов $O$
от координат этого отображения.
\item [Theorem \ref{theorem: coordinates of linear function, octonion}]
зависимость стандартных компонент линейного отображения
алгебры октонионов $O$
от координат этого отображения.
\end{description}

\begin{theorem}
\label{theorem: Standard components of linear function, octonion}
Стандартные компоненты линейной функции
алгебры октонионов $O$ относительно базиса
\EqRef{basis of octonion}
и координаты соответствующего линейного преобразования
удовлетворяют соотношениям
\ShowEq{octonion linear system, 1}
\end{theorem}
\begin{proof}
Пользуясь равенством \EqRef{coordinates of mapping A}
получаем соотношения
\ShowEq{Standard components of linear function, 1, octonion}

Уравнения
\ShowEq{octonion linear system ref, 0}
формируют систему линейных уравнений
\EqRef{octonion linear system, 1, 0}.

Уравнения
\ShowEq{octonion linear system ref, 1}
формируют систему линейных уравнений
\EqRef{octonion linear system, 1, 1}.

Уравнения
\ShowEq{octonion linear system ref, 2}
формируют систему линейных уравнений
\EqRef{octonion linear system, 1, 2}.

Уравнения
\ShowEq{octonion linear system ref, 3}
формируют систему линейных уравнений
\EqRef{octonion linear system, 1, 3}.

Уравнения
\ShowEq{octonion linear system ref, 4}
формируют систему линейных уравнений
\EqRef{octonion linear system, 1, 4}.

Уравнения
\ShowEq{octonion linear system ref, 5}
формируют систему линейных уравнений
\EqRef{octonion linear system, 1, 5}.

Уравнения
\ShowEq{octonion linear system ref, 6}
формируют систему линейных уравнений
\EqRef{octonion linear system, 1, 6}.

Уравнения
\ShowEq{octonion linear system ref, 7}
формируют систему линейных уравнений
\EqRef{octonion linear system, 1, 7}.

\EqRef{octonion, 2, 0} -
это решение системы линейных уравнений
\EqRef{octonion linear system, 1, 0}.
\end{proof}

\begin{theorem}
\label{theorem: octonion, matrix}
Рассмотрим алгебру октонионов $O$ с базисом
\EqRef{basis of octonion}.
Стандартные компоненты линейной функции
и координаты этой функции
удовлетворяют соотношениям
\ShowEq{octonion, 3}
где
\ShowEq{octonion, 3F}
\end{theorem}
\begin{proof}
Запишем систему линейных уравнений
\EqRef{octonion linear system, 1, 0}
в виде произведения матриц
\ShowEq{octonion matrix 0}
Запишем систему линейных уравнений
\EqRef{octonion linear system, 1, 1}
в виде произведения матриц
\ShowEq{octonion matrix 1}
Из равенства \EqRef{octonion matrix 1}
следует
\ShowEq{octonion, 3, 1}
Запишем систему линейных уравнений
\EqRef{octonion linear system, 1, 2}
в виде произведения матриц
\ShowEq{octonion matrix 2}
Из равенства \EqRef{octonion matrix 2}
следует
\ShowEq{octonion, 3, 2}
Запишем систему линейных уравнений
\EqRef{octonion linear system, 1, 3}
в виде произведения матриц
\ShowEq{octonion matrix 3}
Из равенства \EqRef{octonion matrix 3}
следует
\ShowEq{octonion, 3, 3}
Запишем систему линейных уравнений
\EqRef{octonion linear system, 1, 4}
в виде произведения матриц
\ShowEq{octonion matrix 4}
Из равенства \EqRef{octonion matrix 4}
следует
\ShowEq{octonion, 3, 4}
Запишем систему линейных уравнений
\EqRef{octonion linear system, 1, 5}
в виде произведения матриц
\ShowEq{octonion matrix 5}
Из равенства \EqRef{octonion matrix 5}
следует
\ShowEq{octonion, 3, 5}
Запишем систему линейных уравнений
\EqRef{octonion linear system, 1, 6}
в виде произведения матриц
\ShowEq{octonion matrix 6}
Из равенства \EqRef{octonion matrix 6}
следует
\ShowEq{octonion, 3, 6}
Запишем систему линейных уравнений
\EqRef{octonion linear system, 1, 7}
в виде произведения матриц
\ShowEq{octonion matrix 7}
Из равенства \EqRef{octonion matrix 7}
следует
\ShowEq{octonion, 3, 7}
Мы объединяем равенства
\EqRef{octonion matrix 0},
\EqRef{octonion, 3, 1},
\EqRef{octonion, 3, 2},
\EqRef{octonion, 3, 3},
\EqRef{octonion, 3, 4},
\EqRef{octonion, 3, 5},
\EqRef{octonion, 3, 6},
\EqRef{octonion, 3, 7}
в равенстве
\EqRef{octonion, 3, B->A}.
\end{proof}

\begin{theorem}
\label{theorem: coordinates of linear function, octonion}
Стандартные компоненты линейной функции
алгебры октонионов $O$ относительно базиса
\EqRef{basis of octonion}
и координаты соответствующего линейного преобразования
удовлетворяют соотношениям
\ShowEq{octonion, 2}
\end{theorem}
\begin{proof}
Системы линейных уравнений
\EqRef{octonion, 2, 0},
\EqRef{octonion, 2, 1},
\EqRef{octonion, 2, 2},
\EqRef{octonion, 2, 3},
\EqRef{octonion, 2, 4},
\EqRef{octonion, 2, 5},
\EqRef{octonion, 2, 6},
\EqRef{octonion, 2, 7}
получены
в результате перемножения матриц в равенстве
\EqRef{octonion, 3, A->B}.
\end{proof}

Для того, чтобы найти линейное отображение, соответствующее
операции сопряжения, я положу
\ShowEq{octonion conjugation, 1}
Подставив \EqRef{octonion conjugation, 1}
в систему уравнений
\EqRef{octonion, 2, 0},
мы получим
\ShowEq{octonion conjugation, 2}
Следовательно,
\ShowEq{octonion conjugation, 3}

\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\section{Дифференцируемое отображение тела кватернионов}

\begin{theorem}
Если матрица
$\displaystyle
\begin{pmatrix}
\displaystyle\frac{\partial y^{\gi i}}{\partial x^{\gi j}}
\end{pmatrix}
$
является матрица Якоби функции
$
x\rightarrow y
$
тела кватернионов над полем действительных чисел,
то
\ShowEq{quaternion over real field, derivative}
\end{theorem}
\begin{proof}
Следствие теоремы
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: Quaternion over real field}.
\else
\xRef{0701.238}{theorem: Quaternion over real field}.
\fi
\end{proof}

\begin{theorem}
\label{theorem: quaternion conjugation, derivative}
Отображение кватернионов
\[
f(x)=\overline x
\]
имеет производную Гато
\begin{equation}
\label{eq: quaternion conjugation, derivative}
\partial (\overline x)(h)=-\frac 12(h+ihi+jhj+khk)
\end{equation}
\end{theorem}
\begin{proof}
Матрица Якоби отображения $f$ имеет вид
\[
\begin{pmatrix}
1&0&0&0
\\
0&-1&0&0
\\
0&0&-1&0
\\
0&0&0&-1
\end{pmatrix}
\]
Из равенств
\EqRef{quaternion over real field, derivative, 2, 0}
следует
\begin{equation}
\label{eq: quaternion conjugation, derivative, 1}
\StandPartial{y}{x}{00}=
\StandPartial{y}{x}{11}=
\StandPartial{y}{x}{22}=
\StandPartial{y}{x}{33}=
-\frac 12
\end{equation}
Из равенств
\EqRef{quaternion over real field, derivative, 2, 1},
\EqRef{quaternion over real field, derivative, 2, 2},
\EqRef{quaternion over real field, derivative, 2, 3}
следует
\begin{equation}
\label{eq: quaternion conjugation, derivative, 2}
\StandPartial{y}{x}{ij}=0
\ \ \ \gi i\ne\gi j
\end{equation}
Равенство
\EqRef{quaternion conjugation, derivative}
следует из равенств
\EqRef{Gateaux differential, division ring, standard representation},
\EqRef{quaternion conjugation, derivative, 1},
\EqRef{quaternion conjugation, derivative, 2}.
\end{proof}

\begin{theorem}
Сопряжение кватернионов удовлетворяет равенству
\ShowEq{quaternion conjugation}
\end{theorem}
\begin{proof}
Утверждение теоремы следует из теоремы
\ref{theorem: quaternion conjugation, derivative}
и примера \ref{example: differential equation, additive function, division ring}.
\end{proof}

\begin{theorem}
Норма кватерниона удовлетворяет равенствам\footnote{Утверждение
теоремы аналогично примеру X,
\citeBib{Hamilton Elements of Quaternions 1}, с. 455.}
\ShowEq{norm of quaternion, derivative}
\end{theorem}
\begin{proof}
Равенство
\EqRef{norm2 of quaternion, derivative} следует из теоремы
\ref{theorem: quaternion conjugation, derivative}
и равенств \EqRef{norm of quaternion},
\EqRef{Gateaux differential of product, division ring}.
Так как $\NormX\in R$,
то равенство
\EqRef{norm of quaternion, derivative}
следует из равенства
\EqRef{norm2 of quaternion, derivative}.
\end{proof}

\begin{theorem}
Если матрица
$\displaystyle
\begin{pmatrix}
\displaystyle\frac{\partial y^{\gi i}}{\partial x^{\gi j}}
\end{pmatrix}
$
является матрицей Якоби функции
$
x\rightarrow y
$
тела кватернионов над полем действительных чисел,
то
\ShowEq{quaternion over real field, derivative, 1}
\end{theorem}
\begin{proof}
Следствие теоремы
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: octonion, matrix}.
\else
\xRef{0701.238}{theorem: octonion, matrix}.
\fi
\end{proof}
\fi


==> Preface.1003.1544.Russian.tex <==
%auto-ignore
\chapter{Предисловие}

\section{Предисловие к изданию 1}

Когда я приступил к написанию этой книги,
первоначальная задача была довольно простой.
Я собирался переписать содержимое книги
\citeBib{0701.238}, используя аппарат матриц отображений
(\citeBib{1001.4852}).
Однако, мне показалось странным ограничивать себя рассмотрением тела,
когда я понимал, что многие результаты будут верны для
ассоциативной алгебры, а что-то сохранится в случае неассоциативной
алгебры.
Результаты этого исследования будут полезны
для математиков и физиков, которые работают с различными алгебрами,
необязательно ассоциативными.

Когда я записал систему линейных уравнений,
используя матрицы отображений, я понял, что в моих руках
оказался инструмент более мощный, чем я вначале предполагал.
При изучении систем
линейных уравнений мы рассматриваем умножение неизвестной величины,
принадлежащей кольцу или векторному пространству,
на скаляр из соответствующего кольца.
Однако я могу предположить, что неизвестная величина
принадлежат некоторой
универсальной алгебре, имеющей операцию сложения.
Вместо умножения на скаляр я рассматриваю некоторое отображение
универсальной алгебры.
Так возникла теория аддитивных уравнений, которая
во многом похожа на теорию линейных уравнений.

В качестве примера применения новых методов
приведено решение системы линейных уравнений
над полем комплексных чисел при условии, что уравнения содержат
неизвестные величины и величины, сопряжённые им.
Решение подобной системы уравнений подробно рассмотрено
в примере
\ref{example: system of additive equations, complex field}.
Без сомнения, попытка решить систему уравнений
\EqRef{system of additive equations, complex field},
пользуясь определителем, задача непростая.

Переходя к рассмотрению алгебр, я обратил внимание,
что обычно алгебру определяют над полем.
Это видимо необходимо, так как алгебра является векторным пространством.
Однако с точки зрения тех построений, что меня интересуют,
для меня несущественно
является ли алгебра векторным пространством над полем
или свободным модулем над коммутативным кольцом.
Убедившись, что существует исследование алгебр над кольцом,
я решил работать с алгебрами над коммутативным кольцо
при условии, что в случае необходимости я буду ослаблять требования.

На алгебре существует две алгебраические структуры.
Если мы рассматриваем алгебру как кольцо,
то при отображении одной алгебры в другую мы рассматриваем
гомоморфизмы кольца.
Если мы рассматриваем алгебру как модуль над кольцом,
то при отображении одной алгебры в другую мы рассматриваем
линейные отображения.
Очевидно, что если алгебра имеет единицу, то гомоморфизм алгебры
является линейным отображением.
Меня в основном интересуют линейные отображения алгебры.

С того момента, как я рассмотрел тензорное произведение тел
(раздел \xRef{0701.238}{section: Tensor Product of Division Rings}),
меня не оставляло ощущение, что линейное отображение в теле
выражено тензором валентности $2$.
В тоже время было непонятно, каким образом тензор валентности $2$
описывает линейное отображение, хотя для определения
тензора валентности $2$ мне нужно билинейное отображение.

Структура модуля линейных отображений $\mathcal L(A;A)$
определена некоммутативностью произведения в алгебре $A$.
Как только произведение становится коммутативным
я могу вместо выражения $axb$ записать выражение $abx$
и я увижу тензор валентности $1$ там, где вначале был тензор
валентности $2$.

Алгебра $A\otimes A$ - очень интересная алгебра. Формально мне следовало
бы писать $A\otimes A^*$, где $A^*$ - противоположная алгебра.
Однако это привело бы к некоторым проблемам
в записи действия
\begin{equation}
(a\otimes b)\circ x=axb
\label{eq: a b x=axb}
\end{equation}
ибо становится неясно с какой стороны следует писать $b$.
Определение умножения
\[(a\otimes b)\circ(c\otimes d)=(ac)\otimes(db)\]
позволяет сохранить запись \EqRef{a b x=axb}.
Поэтому я предпочёл оставить обозначение $A\otimes A$.

Если алгебра $A$ является свободной конечно мерной ассоциативной алгеброй,
то базис
представления алгебры $A\otimes A$ в модуле $\mathcal L(A;A)$
конечен и позволяет описать все линейные отображения алгебры $A$.

\begin{flushright}
Март, 2010
\end{flushright}

\section{Предисловие к изданию 2}

Вскоре после того как я опубликовал издание 1,
я прочитал мнение профессора Баеза (\citeBib{John Baez: Math Blogs})
где он рассуждал на тему о роли блога в среде математиков.
В частности, Баез порекомендовал посетить сайт
\url{http://www.ncatlab.org/nlab/show/Online+Resources}.
То что я увидел на этой сайт превзошло мои ожидания.

Я провёл немало времени, чтобы понять, какие проблемы в математике интересуют
людей, создавших эту сайт.
Я обратил внимание, что в статье посвящённой
$\Omega$\Hyph группе рассматривается конструкция,
подобная конструкции, рассмотренной у меня в главе
\ref{chapter: Matrix of Mappings}.

Термин $\Omega$\Hyph группа существует только на этой сайт.
На ссылках, которые я имею, речь идёт о группе с операторами,
что соответствует представлению $\Omega$\Hyph алгебры в группе
(обычно записываемой аддитивно).
Поэтому я решил не менять терминологию в этой книге.
Однако я вернусь к этой теме позже.

Меня заинтересовала возможность рассматривать некоммутативное сложение.
Но я встретил проблему определить множество аддитивных отображений.
Я также надеюсь вернуться к этой теме.

\begin{flushright}
Август, 2010
\end{flushright}


==> Quaternion.Russian.tex <==
%auto-ignore
\ifx\PrintBook\undefined
\else
\ePrints{1003.1544}
\ifx\Semafor\ValueOn
\chapter{Алгебра с делением}
\else
\chapter{Алгебра кватернионов}
\label{chapter: Quaternion Algebra}
\fi
\fi

\input{Complex.Number.Russian}

\input{Quaternion.Eq}

\section{Линейная функция алгебры кватернионов}

\begin{theorem}
\label{theorem: Quaternion over real field}
Положим
\ShowEq{basis of quaternion}
базис алгебры кватернионов $H$.
Тогда в базисе \EqRef{basis of quaternion} структурные константы имеют вид
\ShowEq{structural constants, quaternion}
\end{theorem}
\begin{proof}
Значение структурных констант следует из таблицы умножения
\EqRef{product of quaternions}.
\end{proof}

Так как вычисления в этом разделе занимают много места,
я собрал в одном месте ссылки на теоремы в этом разделе.
\begin{description}
\item [Теорема \ref{theorem: Standard components of linear function, quaternion}]
определение координат линейного отображения
алгебры кватернионов $H$
через стандартные компоненты этого отображения.
\item [Равенство \EqRef{quaternion, 3, B->A}]
матричная форма зависимости координат линейного отображения
алгебры кватернионов $H$
от стандартных компонент этого отображения.
\item [Равенство \EqRef{quaternion, 3, A->B}]
матричная форма зависимости стандартных компонент линейного отображения
алгебры кватернионов $H$
от координат этого отображения.
\item [Theorem \ref{theorem: coordinates of linear function, quaternion}]
зависимость стандартных компонент линейного отображения
алгебры кватернионов $H$
от координат этого отображения.
\end{description}

\begin{theorem}
\label{theorem: Standard components of linear function, quaternion}
Стандартные компоненты линейной функции
алгебры кватернионов $H$ относительно базиса
\EqRef{basis of quaternion}
и координаты соответствующего линейного преобразования
удовлетворяют соотношениям
\ShowEq{quaternion linear system, 1}
\end{theorem}
\begin{proof}
Пользуясь равенством
\ePrints{1003.1544}
\ifx\Semafor\ValueOn
\EqRef{coordinates of mapping A}
\else
\EqRef{linear map over field, division ring, relation}
\fi
получаем соотношения
\ShowEq{Standard components of linear function, 1, quaternion}

Уравнения
\ShowEq{quaternion linear system ref, 0}
формируют систему линейных уравнений
\EqRef{quaternion linear system, 1, 0}.

Уравнения
\ShowEq{quaternion linear system ref, 1}
формируют систему линейных уравнений
\EqRef{quaternion linear system, 1, 1}.

Уравнения
\ShowEq{quaternion linear system ref, 2}
формируют систему линейных уравнений
\EqRef{quaternion linear system, 1, 2}.

Уравнения
\ShowEq{quaternion linear system ref, 3}
формируют систему линейных уравнений
\EqRef{quaternion linear system, 1, 3}.
\end{proof}

\begin{theorem}
\label{theorem: Quaternion over real field, matrix}
Рассмотрим алгебру кватернионов $H$ с базисом
\EqRef{basis of quaternion}.
Стандартные компоненты аддитивной функции над полем $F$
и координаты этой функции над полем $F$
удовлетворяют соотношениям
\ShowEq{quaternion, 3}
где
\ShowEq{quaternion, 3, 1}
\end{theorem}
\begin{proof}
Запишем систему линейных уравнений
\EqRef{quaternion linear system, 1, 0}
в виде произведения матриц
\ShowEq{quaternion matrix 0}
Запишем систему линейных уравнений
\EqRef{quaternion linear system, 1, 1}
в виде произведения матриц
\ShowEq{quaternion matrix 1}
Из равенства \EqRef{quaternion matrix 1}
следует
\ShowEq{quaternion over real field, 3, 1}
Запишем систему линейных уравнений
\EqRef{quaternion linear system, 1, 2}
в виде произведения матриц
\ShowEq{quaternion matrix 2}
Из равенства \EqRef{quaternion matrix 2}
следует
\ShowEq{quaternion over real field, 3, 2}
Запишем систему линейных уравнений
\EqRef{quaternion linear system, 1, 3}
в виде произведения матриц
\ShowEq{quaternion matrix 3}
Из равенства \EqRef{quaternion matrix 3}
следует
\ShowEq{quaternion over real field, 3, 3}
Мы объединяем равенства
\EqRef{quaternion matrix 0},
\EqRef{quaternion over real field, 3, 1},
\EqRef{quaternion over real field, 3, 2},
\EqRef{quaternion over real field, 3, 3}
в равенстве
\EqRef{quaternion, 3, B->A}.
\end{proof}

\begin{theorem}
\label{theorem: coordinates of linear function, quaternion}
Стандартные компоненты линейной функции
алгебры кватернионов $H$ относительно базиса
\EqRef{basis of quaternion}
и координаты соответствующего линейного преобразования
удовлетворяют соотношениям
\ShowEq{quaternion over real field}
\end{theorem}
\begin{proof}
Системы линейных уравнений
\EqRef{quaternion over real field, 2, 0},
\EqRef{quaternion over real field, 2, 1},
\EqRef{quaternion over real field, 2, 2},
\EqRef{quaternion over real field, 2, 3}
получены
в результате перемножения матриц в равенстве
\EqRef{quaternion, 3, A->B}.
\end{proof}

\ifx\texFuture\Defined
\section{Отображения между разными алгебрами}

Для алгебры кватернионов над полем действительных чисел
принято обозначение $H=E(R)$.

\begin{theorem}
Линейная функция
\ShowEq{function from R to H}
удовлетворяет равенству
\end{theorem}
\begin{proof}
Над полем действительных чисел
мы можем представить функцию \EqRef{function from R to H}
в виде матрицы
\ShowEq{function from R to H, coordinates}
Если в качестве генератора мы выберем отображение
\ShowEq{function from R to H, generator}
то равенство
\EqRef{linear map, G, coordinates and components, division ring, relation}
принимает вид
\ShowEq{function from R to H, relation}
\end{proof}
\fi

\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\section{Дифференцируемое отображение тела кватернионов}

\begin{theorem}
Если матрица
$\displaystyle
\begin{pmatrix}
\displaystyle\frac{\partial y^{\gi i}}{\partial x^{\gi j}}
\end{pmatrix}
$
является матрица Якоби функции
$
x\rightarrow y
$
тела кватернионов над полем действительных чисел,
то
\ShowEq{quaternion over real field, derivative}
\end{theorem}
\begin{proof}
Следствие теоремы
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: Quaternion over real field}.
\else
\xRef{0701.238}{theorem: Quaternion over real field}.
\fi
\end{proof}

\begin{theorem}
\label{theorem: quaternion conjugation, derivative}
Отображение кватернионов
\[
f(x)=\overline x
\]
имеет производную Гато
\begin{equation}
\label{eq: quaternion conjugation, derivative}
\partial (\overline x)(h)=-\frac 12(h+ihi+jhj+khk)
\end{equation}
\end{theorem}
\begin{proof}
Матрица Якоби отображения $f$ имеет вид
\[
\begin{pmatrix}
1&0&0&0
\\
0&-1&0&0
\\
0&0&-1&0
\\
0&0&0&-1
\end{pmatrix}
\]
Из равенств
\EqRef{quaternion over real field, derivative, 2, 0}
следует
\begin{equation}
\label{eq: quaternion conjugation, derivative, 1}
\StandPartial{y}{x}{00}=
\StandPartial{y}{x}{11}=
\StandPartial{y}{x}{22}=
\StandPartial{y}{x}{33}=
-\frac 12
\end{equation}
Из равенств
\EqRef{quaternion over real field, derivative, 2, 1},
\EqRef{quaternion over real field, derivative, 2, 2},
\EqRef{quaternion over real field, derivative, 2, 3}
следует
\begin{equation}
\label{eq: quaternion conjugation, derivative, 2}
\StandPartial{y}{x}{ij}=0
\ \ \ \gi i\ne\gi j
\end{equation}
Равенство
\EqRef{quaternion conjugation, derivative}
следует из равенств
\EqRef{Gateaux differential, division ring, standard representation},
\EqRef{quaternion conjugation, derivative, 1},
\EqRef{quaternion conjugation, derivative, 2}.
\end{proof}

\begin{theorem}
Сопряжение кватернионов удовлетворяет равенству
\ShowEq{quaternion conjugation}
\end{theorem}
\begin{proof}
Утверждение теоремы следует из теоремы
\ref{theorem: quaternion conjugation, derivative}
и примера \ref{example: differential equation, additive function, division ring}.
\end{proof}

\begin{theorem}
Норма кватерниона удовлетворяет равенствам\footnote{Утверждение
теоремы аналогично примеру X,
\citeBib{Hamilton Elements of Quaternions 1}, с. 455.}
\ShowEq{norm of quaternion, derivative}
\end{theorem}
\begin{proof}
Равенство
\EqRef{norm2 of quaternion, derivative} следует из теоремы
\ref{theorem: quaternion conjugation, derivative}
и равенств \EqRef{norm of quaternion},
\EqRef{Gateaux differential of product, division ring}.
Так как $\NormX\in R$,
то равенство
\EqRef{norm of quaternion, derivative}
следует из равенства
\EqRef{norm2 of quaternion, derivative}.
\end{proof}

\begin{theorem}
Если матрица
$\displaystyle
\begin{pmatrix}
\displaystyle\frac{\partial y^{\gi i}}{\partial x^{\gi j}}
\end{pmatrix}
$
является матрицей Якоби функции
$
x\rightarrow y
$
тела кватернионов над полем действительных чисел,
то
\ShowEq{quaternion over real field, derivative, 1}
\end{theorem}
\begin{proof}
Следствие теоремы
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: Quaternion over real field, matrix}.
\else
\xRef{0701.238}{theorem: Quaternion over real field, matrix}.
\fi
\end{proof}
\fi

\ePrints{1003.1544}
\ifx\Semafor\ValueOff
\begin{theorem}
Мы можем отождествить кватернион
\ShowEq{quaternion a}
и матрицу
\ShowEq{quaternion product ax, Jacobian}
\end{theorem}
\begin{proof}
Произведение кватернионов
\EqRef{quaternion a} и
\ShowEq{quaternion x}
имеет вид
\ShowEq{quaternion product ax}
Следовательно, функция $f_a(x)=ax$ имеет матрицу Якоби
\EqRef{quaternion product ax, Jacobian}.
Очевидно, что $f_a\circ f_b=f_{ab}$. Аналогичное равенство
верно для матриц
\ShowEq{quaternion ab, Jacobian product}
Следовательно, мы можем отождествить кватернион $a$ и матрицу $J_a$.
\end{proof}
\fi


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%A%0
\Symb%
   {$(^a_b)$\hyph\CR квазидетерминант}%
   {a b CR quasideterminant definition}%
\Symb%
   {минор}%
   {A from b a}%
\Symb%
   {минор}%
   {A from columns T}%
\Symb%
   {минор}%
   {A from rows S}%
\Symb%
   {минор}%
   {A without column a}%
\Symb%
   {минор}%
   {A without columns T}%
\Symb%
   {минор}%
   {A without row b}%
\Symb%
   {минор}%
   {A without rows S}%
\Symb%
   {аффинное пространство}%
   {affine space, division ring}%
\Symb%
   {аффинное пространство}%
   {An}%
\Symb%
   {ассоциатор $R$\Hyph алгебры}%
   {associator of algebra}%
\Symb%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb%
   {коммутатор $R$\Hyph алгебры}%
   {commutator of algebra}%
\Symb%
   {компонента линейного отображения $\Vector{A}$ $D$\Hyph векторного пространства}%
   {component of linear map, D vector space}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb%
   {\drc вектор}%
   {drc vector}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
\Symb%
   {лупа автоморфизмов представления $f$}%
   {loop of automorphisms of representation}%
\Symb%
   {норма отображения $\Vector A$ нормированного $D$\hyph векторного пространства}%
   {norm of map, D vector space}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb%
   {частное линейное отображение переменной $v^i$}%
   {partial linear map of variable}%
\Symb%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
\Symb%
   {множество линейных отображений тела $D_1$ в тело $D_2$}%
   {set linear maps, division ring}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb%
   {стандартная компонента тензора в тензорном произведении алгебр}%
   {standard component of tensor, algebra}%
\Symb%
   {правый сдвиг}%
   {starT shift}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb%
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Symb%
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Symb%
   {левый сдвиг}%
   {Tstar shift}%
\Symb%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов \rcd векторного пространства $\mathcal{V}$}%
   {basis manifold of rcd vector space}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb%
   {многообразие базисов представления $f$}%
   {basis manifold representation F algebra}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb%
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power A of bundle B}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb%
   {многообразие \drc базисов аффинного пространства}%
   {drc Basis Manifold, Affine Space, division ring}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
\Symb%
   {структура всех подпредставлений представления $f$}%
   {lattice of subrepresentations}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, 1 n}%
\Symb%
   {структурные константы алгебры $A$ над кольцом $R$}%
   {structural constants of algebra}%
\Symb%
   {структурные константы тела $D$ над полем $F$}%
   {structural constants of division ring over field}%

\SetIndexSpace%C%0
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли}%
   {basis vector of representation of Lie group}%
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
\Symb%
   {координаты базового вектора представления группы Ли}%
   {basis vector of representation of Lie group, coordinates}%
\Symb%
   {компонента производной Гато отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of map, algebra}%
\Symb%
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space}%
\Symb%
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, division ring}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of Second Order, algebra}%
\Symb%
   {компонента производной Гато второго порядка отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$ тела}%
   {component of Gateaux derivative of Second Order, division ring}%
\Symb%
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in bundle, 1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
\Symb%
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$ алгебры}%
   {Gateaux derivative of map, algebra}%
\Symb%
   {производная Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, division ring}%
\Symb%
   {производная Гато отображения $f$ алгебры}%
   {Gateaux derivative of map, fraction, algebra}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, algebra}%
\Symb%
   {производная Гато второго порядка отображения $\Vector f$}%
   {Gateaux derivative of Second Order, D vector space}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, division ring}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
\Symb%
   {дифференциал Гато отображения $f$ алгебры}%
   {Gateaux differential of map, algebra}%
\Symb%
   {дифференциал Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux differential of map, D vector space}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, division ring}%
\Symb%
   {дифференциал Гато второго порядка отображения $f$ алгебры}%
   {Gateaux differential of Second Order, algebra}%
\Symb%
   {дифференциал Гато второго порядка отображения $\Vector f$}%
   {Gateaux differential of Second Order, D vector space}%
\Symb%
   {дифференциал Гато второго порядка отображения $f$ тела}%
   {Gateaux differential of Second Order, division ring}%
\Symb%
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 1, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 2, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 3, D vector space}%
\Symb%
   {смешанная частная производная Гато отображения $f^j$ по переменным $v^i$, $v^j$}%
   {Gateaux partial derivative of Second Order, D vector space}%
\Symb%
   {частная производная Гато отображения $f^j$ по переменной $v^i$}%
   {Gateaux partial derivative, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 1, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 2, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 3, D vector space}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb%
   {производная Картана}%
   {overbrace D}%
\Symb%
   {производная}%
   {overline D}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
\Symb%
   {\drc векторное пространство \subs строк}%
   {r rows drc vector space}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
\Symb%
   {стандартная компонента производной Гато отображения $f$}%
   {standard component of Gateaux derivative, algebra}%
\Symb%
   {стандартная компонента дифференциала Гато отображения $f$}%
   {standard component of Gateaux differential, division ring}%
\Symb%
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Symb%
   {тензорное произведение колец}%
   {tensor product of rings}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%E%0
\Symb%
   {аффинный базис}%
   {Affine Basis}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
\Symb%
   {базис в векторном пространстве $\mathcal{V}$}%
   {basis in V}%
\Symb%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb%
   {аффинный базис}%
   {drc affine basis, division ring}%
\Symb%
   {базис в \Drc векторного расслоения}%
   {drc basis, vector bundle}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\mathcal{E}$}%
   {set of starT nonsingular transformations of bundle}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\mathcal{E}$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%F%0
\Symb%
   {активное представление лупы $\mathfrak A(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Symb%
   {координаты базиса в \rcd векторном пространстве \sups строк}%
   {basis coordinates, c rows rcd vector space}%
\Symb%
   {координаты базиса в \drc векторном пространстве \subs строк}%
   {basis coordinates, r rows drc vector space}%
\Symb%
   {базис в \rcd векторного пространства \sups строк}%
   {basis, c rows rcd vector space}%
\Symb%
   {базис в \drc векторном пространстве \subs строк}%
   {basis, r rows drc vector space}%
\Symb%
   {центро-аффинный}%
   {Central Affine Basis, division ring}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Symb%
   {компонента полилинейного отображения тела}%
   {component of polylinear map, division ring}%
\Symb%
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb%
   {норма отображения в $D$\Hyph алгебру}%
   {norm of map, algebra}%
\Symb%
   {норма отображения $f$  тела}%
   {norm of map, division ring}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of Tstar representation of group}%
\Symb%
   {ортонормальный базис}%
   {Orthonornal Basis, division ring}%
\Symb%
   {система отсчёта}%
   {reference frame}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
\Symb%
   {стандартная $F$\Hyph компонента линейного отображения $f$ }%
   {standard component of linear map, division ring}%
\Symb%
   {стандартная компонента полилинейного отображения $f$ тела}%
   {standard component of polylinear map, division ring}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor, division ring}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb%
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb%
   {алгебра Ли группы Ли}%
   {g}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb%
   {группа гомоморфизмов векторного пространства $\mathcal{V}$}%
   {GV}%
\Symb%
   {малая группа элемента $x$}%
   {little group}%
\Symb%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective covariant starT representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective covariant starT representation of group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective covariant Tstar representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective covariant Tstar representation of group}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, 1 n}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb%
   {алгебра кватернионов над полем действительных чисел}%
   {quaternion algebra over real field}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%

\SetIndexSpace%K%0
\Symb%
   {ядро линейного отображения $D$\Hyph векторного пространства}%
   {kernel of linear map, D vector space}%
\Symb%
   {ядро линейного отображения тела}%
   {kernel of linear map, division ring}%

\SetIndexSpace%L%0
\Symb%
   {левый сдвиг}%
   {left shift}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb%
   {предел последовательности в нормированном кольце}%
   {limit of sequence, normed ring}%
\Symb%
   {предел последовательности в нормированном теле}%
   {limit of sequence, valued division ring}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
\Symb%
   {\rcd векторное пространство \drc линейных отображений \drc векторного пространства $\Vector V$ в \drc векторное пространство $\Vector W$}%
   {set drc linear maps, drc vector space}%
\Symb%
   {множество линейных отображений алгебры $A_1$ в алгебру $A_2$}%
   {set linear mappings, algebra}%
\Symb%
   {множество линейных отображений $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector{W}$}%
   {set linear maps, D vector space}%
\Symb%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$  в модуль $S$}%
   {set polylinear mappings, algebra}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
\Symb%
   {\drc векторное пространство \rcd линейных отображений \rcd векторного пространства $\Vector{V}$ в \rcd векторное пространство $\Vector{W}$}%
   {set rcd linear maps, rcd vector space}%
\Symb%
   {множество \sT представлений тела $S$ в аддитивной группе тела $R$}%
   {set sT representations, division ring}%
\Symb%
   {множество \Ts представлений тела $S$ в аддитивной группе тела $R$}%
   {set Ts representations, division ring}%

\SetIndexSpace%M%0
\Symb%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb%
   {множество преобразований множества $M$}%
   {set of transformations}%
\Symb%
   {множество \Ts преобразований множества $M$}%
   {set of Tstar transformations}%
\Symb%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%N%0
\Symb%
   {ядро $R$\Hyph алгебры $A$}%
   {nucleus of algebra}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
\Symb%
   {орбита представления расслоенной группы $\mathcal{G}$}%
   {orbit of representation of fibered group}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
\Symb%
   {\rcd векторное пространство \sups строк}%
   {c rows rcd vector space}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in reduced bundle, 2}%
\Symb%
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb%
   {правый сдвиг}%
   {right shift}%
\Symb%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%
\Symb%
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%

\SetIndexSpace%T%0
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Symb%
   {касательная плоскость к группе $G$}%
   {TaG}%

\SetIndexSpace%V%0
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Symb%
   {\dcr векторное пространство}%
   {left CR vector space}%
\Symb%
   {\drc векторное пространство}%
   {left RC vector space}%
\Symb%
   {\crd векторное пространство}%
   {right CR vector space}%
\Symb%
   {\rcd векторное пространство}%
   {right RC vector space}%
\Symb%
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Symb%
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Symb%
   {векторное пространство}%
   {V}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J_f(X)$}%
   {coordinate set of representation}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Symb%
   {координаты пассивного отображения многообразия базисов представления}%
   {coordinates of passive map of basis manifold of representation}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%

\SetIndexSpace%X%0
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
\Symb%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%Z%0
\Symb%
   {центр $R$\Hyph алгебры $A$}%
   {center of algebra}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
\Symb%
   {связность}%
   {conection overline}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%

\SetIndexSpace%Fi%2
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%Phi%2
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%Pi%2
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
\Symb%
   {произведение групп $G_i$, $i\in I$}%
   {product of groups}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, i 1 n}%
\Symb%
   {произведением объектов $\{B_i,i\in I\}$ в категории $\mathcal A$}%
   {product of objects in category}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, i 1 n}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%S%2
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb%
   {подрасслоение}%
   {subbundle}%

\CloseIndex


==> Tensor.Algebra.Russian.tex <==
%auto-ignore
\input{Tensor.Algebra}

%\chapter{Тензорное произведение}

\section{Тензорное произведение алгебр}

\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOff
\begin{definition}
\label{definition: polylinear map of modules}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Мы будем называть отображение
\ShowEq{polylinear map of algebras}
\AddIndex{полилинейным отображением модулей}
{polylinear map of modules}
$A_1$, ..., $A_n$
в модуль $S$,
если
\ShowEq{polylinear map of algebras, 1}
\qed
\end{definition}

\begin{definition}
\label{definition: polylinear map of algebras}
Пусть $D$ - коммутативное ассоциативное кольцо.
Пусть $A_1$, ..., $A_n$ -
$D$\Hyph алгебры и $S$ - $D$\Hyph модуль.
Мы будем называть отображение
\ShowEq{polylinear map of algebras}
\AddIndex{полилинейным отображением алгебр}
{polylinear map of algebras}
$A_1$, ..., $A_n$
в модуль $S$,
если
\ShowEq{polylinear map of algebras, 1}
Обозначим
\ShowEq{set polylinear mappings, algebra}
множество полилинейных отображений
алгебр
$A_1$, ..., $A_n$
в модуль
$S$.
\qed
\end{definition}

\begin{definition}
\label{definition: tensor product of algebras}
Пусть $A_1$, ..., $A_n$ -
свободные алгебры над  коммутативным кольцом $D$.\footnote{Я определяю
тензорное произведение алгебр
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.}
Рассмотрим категорию $\mathcal A$ объектами которой являются
полилинейные над коммутативным кольцом $D$ отображения
\ShowEq{polylinear mappings category}
где $S_1$, $S_2$ - модули над кольцом $D$.
Мы определим морфизм $f\rightarrow g$
как линейное над коммутативным кольцом $D$ отображение $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{polylinear mappings category, diagram}
Универсальный объект
\ShowEq{tensor product of algebras}
категории $\mathcal A$
называется \AddIndex{тензорным произведением алгебр $A_1$, ..., $A_n$}
{tensor product of algebras}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: tensor product of algebras is module}
Тензорное произведение алгебр существует.
\end{theorem}
\begin{proof}
Пусть $M$ - модуль над кольцом $D$, порождённый
произведением $\Times$
алгебр $A_1$, ..., $A_n$.
Инъекция
\ShowEq{map i, algebra, tensor product, 1}
определена по правилу
\ShowEq{map i, algebra, tensor product}
Пусть $N\subset M$ - подмодуль, порождённый элементами вида
\ShowEq{kernel, algebra, tensor product}
где $d_i\in A_i$, $c_i\in A_i$, $a\in D$.
Пусть
\[
j:M\rightarrow M/N
\]
каноническое отображение на фактормодуль.
Рассмотрим коммутативную диаграмму
\ShowEq{diagram top, algebra, tensor product}
Поскольку элементы \EqRef{kernel 1, algebra, tensor product}
и \EqRef{kernel 2, algebra, tensor product}
принадлежат ядру линейного отображения $j$,
то из равенства
\EqRef{map i, algebra, tensor product}
следует
\ShowEq{f, algebra, tensor product}
Из равенств \EqRef{f 1, algebra, tensor product}
и \EqRef{f 2, algebra, tensor product}
следует, что отображение $f$ полилинейно над кольцом $D$.
Поскольку $M$ - модуль с базисом
$\Times$, то, согласно теореме \citeBib{Serge Lang}-1
на с. 104,
для любого модуля $V$ и любого
полилинейного над $D$ отображения
\ShowEq{diagram bottom, 1, algebra, tensor product}
существует единственный гомоморфизм $k:M\rightarrow V$,
для которого коммутативна следующая диаграмма
\ShowEq{diagram bottom, algebra, tensor product}
Так как $g$ - полилинейно над $D$, то
\ShowEq{ker k subseteq N}
Согласно утверждению 
на с. \citeBib{Serge Lang}-94,
отображение $j$ универсально в категории гомоморфизмов
векторного пространства $M$,
ядро которых содержит $N$.
Следовательно, определён гомоморфизм
\[
h:M/N\rightarrow V
\]
для которого коммутативна диаграмма
\begin{equation}
\label{eq: diagram right, algebra, tensor product}
\xymatrix{
&M/N\ar[dd]^h
\\
M\ar[dr]^k\ar[ur]_j
\\
&V
}
\end{equation}
Объединяя диаграммы
\EqRef{diagram top, algebra, tensor product},
\EqRef{diagram bottom, algebra, tensor product},
\EqRef{diagram right, algebra, tensor product},
получим коммутативную диаграмму
\ShowEq{diagram, algebra, tensor product}
Так как $\mathrm{Im}f$ порождает $M/N$,
то отображение $h$ однозначно определено.
\end{proof}

Согласно доказательству теоремы
\ref{theorem: tensor product of algebras is module}
\[A_1\otimes...\otimes A_n=M/N\]
Для $d_i\in A_i$ будем записывать
\ShowEq{map j, algebra, tensor product}

\begin{theorem}
\label{theorem: tensor product and polylinear mapping}
Пусть $A_1$, ..., $A_n$ -
алгебры над коммутативным кольцом $D$.
Пусть
\ShowEq{map f, 1, algebra, tensor product}
полилинейное отображение, определённое равенством
\ShowEq{map f, algebra, tensor product}
Пусть
\ShowEq{map g, algebra, tensor product}
полилинейное отображение в $D$\Hyph модуль $V$.
Существует $D$\Hyph линейное отображение
\ShowEq{map h, algebra, tensor product}
такое, что диаграмма
\ShowEq{map gh, algebra, tensor product}
коммутативна.
\end{theorem}
\begin{proof}
Равенство
\EqRef{map f, algebra, tensor product}
следует
из равенств
\EqRef{map i, algebra, tensor product} и
\EqRef{map j, algebra, tensor product}.
Существование отображения $h$ следует из определения
\ref{definition: tensor product of algebras}
и построений, выполненных при доказательстве теоремы
\ref{theorem: tensor product of algebras is module}.
\end{proof}

Равенства \EqRef{f 1, algebra, tensor product}
и \EqRef{f 2, algebra, tensor product}
можно записать в виде
\ShowEq{tensors, algebra, tensor product}

\begin{theorem}
\label{theorem: tensor product and product in algebra}
Пусть $A$ -
алгебра над коммутативным кольцом $D$.
Существует линейное отображение
\ShowEq{tensor product and product in algebra}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: tensor product and polylinear mapping}
и определения
\ref{definition: algebra over ring}.
\end{proof}
\else
\newpage
Для $a_i\in A_i$, $i=1$, ..., $n$,
$a_1\otimes...\otimes a_n\in A_1\otimes...\otimes A_n$.
Согласно определению
\ShowEq{tensors, algebra, tensor product}

\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\newpage
\fi
\begin{remark}
\label{remark: representation of tensor, ring}
Представление тензора в виде
\ShowEq{tensor representation, algebra}
неоднозначно.
Если $r\in D$, то
\[
(d_1 r)
\otimes
d_2
=d_1
\otimes
(rd_2 )
\]
Чисто алгебраическими методами мы можем
увеличить либо уменьшить число слагаемых.
К числу допустимых преобразований относится
\begin{align*}
&d_1
\otimes
d_2
+c_1
\otimes
c_2
\\
=&d_1
\otimes
(d_2-c_2+c_2)
+c_1
\otimes
c_2
\\
=&d_1
\otimes
(d_2-c_2)
+d_1
\otimes
c_2
+c_1
\otimes
c_2
\\
=&d_1
\otimes
(d_2-c_2)
+(d_1
+c_1)
\otimes
c_2
\end{align*}
\qed
\end{remark}
\fi

\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\newpage
\fi
\begin{theorem}
\label{theorem: standard component of tensor, division ring}
Тензорное произведение $\Tensor A$ свободных
конечномерных алгебр
$A_1$, ..., $A_n$
над коммутативным кольцом $D$ является свободной
конечномерной алгеброй.

Пусть
\ShowEq{tensor product of algebras, basis i}
- базис алгебры $A_i$ над кольцом $D$.
Произвольный тензор $a\in\Tensor A$ можно представить в виде
\ShowEq{tensor canonical representation, algebra}
%Выражение \EqRef{tensor canonical representation, algebra}
%определенно однозначно с точностью до выбора базиса.
Мы будем называть выражение
$\ShowSymbol{standard component of tensor, algebra}$
\AddIndex{стандартной компонентой тензора}
{standard component of tensor, algebra}.
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Алгебры
$A_1$, ..., $A_n$
являются модулями над кольцом $D$.
Согласно теореме
\ref{theorem: tensor product of algebras is module},
$\Tensor A$ является модулем. 

Вектор $a_i\in A_i$ имеет разложение
\ShowEq{expansion i relative basis}
относительно базиса $\Basis e_i$.
Из равенств
\EqRef{tensors 1, algebra, tensor product},
\EqRef{tensors 2, algebra, tensor product}
следует
\ShowEq{expansion i relative basis, 1}
Так как множество тензоров $\Tensor a$
является множеством образующих модуля $\Tensor A$,
то тензор
$a\in\Tensor A$
можно записать в виде
\ShowEq{tensor canonical representation 1, algebra}
где
\ShowEq{tensor canonical representation 2, algebra}
Положим
\ShowEq{tensor canonical representation 3, algebra}
Тогда равенство \EqRef{tensor canonical representation 1, algebra}
примет вид
\EqRef{tensor canonical representation, algebra}.

Следовательно, множество тензоров $\TensorBasis i$
является множеством образующих модуля $\Tensor A$.
Так как размерность модуля $A_i$, $i=1$, ..., $n$, конечна,
то конечно множество тензоров $\TensorBasis i$.
Следовательно, множество тензоров $\TensorBasis i$
содержит базис модуля $\Tensor A$, и модуль $\Tensor A$
является свободным модулем над кольцом $D$.

Мы определим произведение тензоров типа $\Tensor a$ покомпонентно
\ShowEq{product of tensors, algebra, tensor product}
В частности, если для любого $i$, $i=1$, ..., $n$,
$a_i\in A_i$ имеет обратный,
то тензор
\ShowEq{inverse tensor, algebra, 1}
имеет обратный
\ShowEq{inverse tensor, algebra, 2}

Определение произведения
\EqRef{product of tensors, algebra, tensor product}
согласовано с равенством
\EqRef{tensors 2, algebra, tensor product}
так как
\ShowEq{product of tensors, algebra, tensor product, 1}
Из равенства
\EqRef{tensors 1, algebra, tensor product}
следует дистрибутивность умножения по отношению к сложению
\ShowEq{product of tensors, algebra, tensor product, 2}
Равенство
\EqRef{product of tensors, algebra, tensor product, 2}
позволяет определить произведение для любых тензоров $a$, $b$.
\end{proof}

\begin{remark}
\label{remark: tensor product of algebras}
Согласно замечанию
\ref{remark: opposite algebra},
мы можем определить различные структуры алгебры
в тензорном произведении алгебр.
Например, алгебры $A_1\otimes A_2$,
$A_1\otimes A_2^*$, $A_1^*\otimes A_2$
определены на одном и том же модуле.
\qed
\end{remark}
\fi

\begin{theorem}
Пусть $\Basis e_i$ - базис алгебры $A_i$ над кольцом $D$.
Пусть $B_{i\cdot}{}^{\gi j}_{\gi{kl}}$ -
структурные константы алгебры $A_i$ относительно базиса $\Basis e_i$.
Структурные константы тензорного произведение $\Tensor A$
относительно базиса $\TensorBasis i$ имеют вид
\ShowEq{structural constants tensor algebra}
\ePrints{Presentation.1006.2597}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Непосредственное перемножение тензоров
$\TensorBasis i$ имеет вид
\ShowEq{structural constants tensor algebra, proof, 1}
Согласно определению структурных констант
\ShowEq{structural constants tensor algebra, proof, 2}
Равенство
\EqRef{structural constants tensor algebra}
следует из сравнения
\EqRef{structural constants tensor algebra, proof, 1},
\EqRef{structural constants tensor algebra, proof, 2}.

Из цепочки равенств
\ShowEq{structural constants tensor algebra, proof, 3}
следует, что определение произведения
\EqRef{structural constants tensor algebra, proof, 2}
со структурными константами
\EqRef{structural constants tensor algebra}
согласовано с определением произведения
\EqRef{product of tensors, algebra, tensor product}.
\end{proof}

\begin{theorem}
Для тензоров $a$, $b\in\Tensor A$
стандартные компоненты произведения удовлетворяют равенству
\ShowEq{standard components of product, tensor product}
\end{theorem}
\begin{proof}
Согласно определению
\ShowEq{standard components of product, tensor product, 1}
В тоже время
\ShowEq{standard components of product, tensor product, 2}
Равенство
\EqRef{standard components of product, tensor product}
следует из равенств
\EqRef{standard components of product, tensor product, 1},
\EqRef{standard components of product, tensor product, 2}.
\end{proof}

\begin{theorem}
Если алгебра $A_i$, $i=1$, ..., $n$, ассоциативна,
то тензорное произведение $\Tensor A$ - ассоциативная алгебра.
\end{theorem}
\begin{proof}
Поскольку
\ShowEq{tensor product, associative algebra, 1}
то
\ShowEq{tensor product, associative algebra, 2}
\end{proof}
\fi
